CAMETA: Conflict-Aware Multi-Agent Estimated Time of Arrival Prediction for Mobile Robots

This study presents the conflict-aware multi-agent estimated time of arrival (CAMETA) framework, a novel approach for predicting the arrival times of multiple agents in unstructured environments without predefined road infrastructure. The CAMETA framework consists of three components: a path planning layer generating potential path suggestions, a multi-agent ETA prediction layer predicting the arrival times for all agents based on the paths, and lastly, a path selection layer that calculates the accumulated cost and selects the best path. The novelty of the CAMETA framework lies in the heterogeneous map representation and the heterogeneous graph neural network architecture. As a result of the proposed novel structure, CAMETA improves the generalization capability compared to the state-of-the-art methods that rely on structured road infrastructure and historical data. The simulation results demonstrate the efficiency and efficacy of the multi-agent ETA prediction layer, with a mean average percentage error improvement of 29.5% and 44% when compared to a traditional path planning method (A *) which does not consider conflicts. The performance of the CAMETA framework shows significant improvements in terms of robustness to noise and conflicts as well as determining proficient routes compared to state-of-the-art multi-agent path planners.

==> LargeObjects/CostResultTable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\caption{Comparison of the overall path planning framework }
\label{table:comparisonPathplanning}
\resizebox{0.98\textwidth}{!}{
    \begin{tabular}{|c|cc|cc|cc|cc|}
    \hline
    \multirow{2}{*}{Global planner} &
    \multicolumn{2}{c|}{Noise level: 0\%}&
    \multicolumn{2}{c|}{Noise level: 0.0001\%}&
    \multicolumn{2}{c|}{Noise level: 0.001\%}&
    \multicolumn{2}{c|}{Noise level: 0.01\%} \\&
    \multicolumn{1}{l}{Makespan} & \multicolumn{1}{l|}{Sum of costs} &
    \multicolumn{1}{l}{Makespan} & \multicolumn{1}{l|}{Sum of costs} &
    \multicolumn{1}{l}{Makespan} & \multicolumn{1}{l|}{Sum of costs} &
    \multicolumn{1}{l}{Makespan} & \multicolumn{1}{l|}{Sum of costs} \\ \hline \hline
    A*
        & 262.0
        & 50282.0
        & 262.76
        & 50294.36
        & 267.4
        & 50394.84
        & 273.64
        & 50949.6
    \\ 
    \rowcolor{lightgray}PIBT
        & 273.0
        & \textbf{48628.0}
        & 273.0
        & \textbf{49236.76}
        & 277.4
        & 51194.24
        & 288.0
        & 54387.8
    \\ 
    CAMAETA
        & 260.0
        & 49823.0
        & 260.88
        & 49810.16
        & 261.84
        & \textbf{49742.2}
        & 271.4
        & \textbf{50301.8}
    \\
    \hline\hline
    \rowcolor{lightgray}CBS
        & 266.0
        & 46113.0
        & 267.12
        & 46336.2
        & 279.24
        & 47610.08
        & 292.68
        & 50129.76
    \\ \hline
    \end{tabular}
}
\end{table*}

==> old_icra/abstract.tex <==
This study proposes a conflict-aware multi-agent global planner (CAMAGP) framework, which consists of a novel heterogeneous map representation, traditional path planning algorithm, and novel heterogeneous graph neural network architecture for multi-agent arrival time estimation. Instead of relying on the structured road infrastructure and historical data to predict the time of arrival, the proposed framework benefits from the total path length and basic structural features, which has better generalization capability. To the best of our knowledge, this work is the first attempt to predict multi-agent arrival times without any structured road infrastructure. The extensive simulation results illustrate the accuracy and efficacy of the proposed method, demonstrating its feasibility and effectiveness. Compared to a naive method that does not consider conflict, the best-trained iterative multi-step model improves the overall mean average percentage error by 29.5\%, while the best direct multi-step model improves by 44\%.



% %As the popularity of autonomous mobile robot applications is rising in the industry, conflict-aware multi-agent path planning becomes essential for a smooth and efficient operation of autonomous robots in highly dynamic environments.
% This study proposes a framework for a Conflict Aware Multi-Agent Global Planner (CAMAGP), which combines novel heterogeneous map representation, traditional path-planning algorithms, and a novel heterogeneous graph neural network architecture for multi-agent arrival time estimation. 
% % The proposed framework relies not on historical data but on naive path distance along with the structural features of the path. As a result, the framework does not depend on structured road infrastructure in order to predict the arrival time.
% Contrary to other methods, which rely on structured road infrastructure and historical data to predict the time of arrival, the proposed framework only relies on the total path length and basic structural features, thus making it more general in its application.
% % Since the proposed framework does not rely on historical data but uses naive path distance and structural features of the path, the framework does not depend on a structured road infrastructure to predict the arrival time.
% To the best of our knowledge, this work is the first attempt to predict multi-agent arrival times without any structured road infrastructure. 
% Compared to a naive method that does not consider conflict, the best trained iterative multi-step model improves the overall mean average percentage error by 29.5\%, while the best direct multi-step model improves by 44\%.
% The results illustrate the accuracy and efficacy of the proposed method, demonstrating its feasibility and effectiveness.

% % NOTE:
% % Since the first sentence of the paragraph will be deleted, you will have some extra space in your abstract. How about keeping this sentence but adding a few details to your results by adding one more sentence before this sentence? you can write one or two significant discussions for your results. For example: 
% % "The best trained IMS model improves the average MAPE by 29.5% compared to the naive method, while the best DMS model improves by 44%"


==> old_icra/backup.tex <==
\section{Introduction}
\label{sec:introduction}
As part of industrial 4.0 and the need for flexible and efficient manufacturing, transportation and logistics, companies increasingly rely on autonomous mobile robots to handle and distribute resources. A key component to successfully implement applications of large scale robots is to handle collision-free multi-agent path planning and control the flow of robots in the system. Many research efforts have been devoted to this field in recent years from different perspectives.
\smallbreak
% Decentralised vs centralised
A multi-agent system can generally be categorised into two architectures: a centralised or decentralised system. In a centralised system, all robots transmit information to a centralised ground station. The ground station processes all the robots intentions and sends a collision-free path back to the robot \cite{CBS_paper}. While centralised systems have many benefits, in practice, centralised systems heavily depend on powerful machines and a fast communication network, which is costly to be deployed in large scale environments with a large number of robots.
In a decentralised system, each robot computes its own path through the environment, creating a more scalable solution compared to the centralised system. However, the problem is the complexity of predicting the flow of the environment as a whole, as each robot might not have access to the entire state space of the system.
\medbreak
% Local planning and global planning
For many decades, researchers have developed many different ideas on how to solve the decentralised collision-free path for a robot with incomplete environment information. Many papers have succeeded in optimising this\cite{Mapper}\cite{MAG_planner}, but these methods only optimise the flow on a very local level, without considering the flow on a global level. In this paper, we focus on optimising a decentralised global planner, considering not only the distance of the planned path but also the traffic flow throughout the planned time. Inspired by the state-of-the-art estimated time of arrival method \cite{GOOGLE_ETA}, we utilise \ac{GNN} for estimating the flow of the system and predict better trajectories than the naive shortest route. We will concentrate on the decentralised system, where limited communication is available, and we do not have perfect information about the other robots. The solution needs to predict the movement of other robots in the system in order to maximise the flow. 
\begin{figure}[t]
    \centering
    \includesvg[width=0.49\textwidth]{images/introduction/Method_overview.svg}
    \caption{Method overview: Explanation is coming up}
    \label{fig:overview}
\end{figure}

\textcolor{red}{Contributions}
\noindent The major contributions of this study are the followings:
\begin{itemize}
    \item First, we investigate the global multi-agent path planning problem in highly active industrial environments. To model these environments and locate the potential bottle-neck areas, we propose an automatic bottle-neck detection and topological graph construction method from 2d occupancy grid maps.
    \item Secondly, we propose a decentralized global planner utilizing graph neural networks for multi-robot environments for optimizing flow in industrial scenarios.
    \item Finally,  
\end{itemize}
The rest of this paper is organised as follows. 
Section \ref{sec:related_work} introduces the state-of-the-art in the field of multi-agent path-planning and global path planning. Section \ref{sec:methodology} provides some preliminaries for our problem formulation along with the approach of our \ac{DMAGGPP} for generalised indoor industrial environments. Section \ref{sec:experiments} explains the experiment setup followed by the results of \ac{DMAGGPP} in various grid world environments which is presented in section \ref{sec:results}. Finally, we give a brief conclusion in section \ref{sec:conclusion}.





==> old_icra/conclusion.tex <==
\section{Conclusion and future work}
\label{sec:conclusion}
% In this work, we conduct pioneering research by developing a framework for predicting conflicts and estimating the time of arrival in a multi-agent environment. We formulate our problem as a spatio-temporal graph focusing on edge prediction. This allows for the estimated time of arrival prediction of all robots simultaneously, which previous work has not been able to accomplish. While this is the first study in the field on systemwide estimated time of arrival, it has been demonstrated to increase the accuracy of the predicted time of arrival. As a result, the overall framework's capacity to accurately evaluate the cost of each route improves. 

In this work, we develop a framework to predict conflicts and estimate the time of arrival in multi-agent environments. We formulate our problem as a spatio-temporal graph focusing on edge prediction. The proposed methodology allows the estimated time of arrival prediction of all robots simultaneously, which was not possible by the previously published works. While this is the first study on the system-wide estimated time of arrival, we also demonstrate to increase in the accuracy of the predicted time of arrival. 

% In future work, a couple of features could be incorporated into the current framework. Firstly, incorporate robot acceleration to reflect the real-world dynamics more accurately. Secondly, include multiple types of robots. As we are representing the problem as a heterogeneous graph, incorporating dynamics, constraints, and different types of robots into nodes is very feasible. 
As future work, we plan to incorporate robot acceleration to reflect real-world dynamics more accurately. We will also include multiple types of robots in the same environment. As we represent the problem as a heterogeneous graph, incorporating dynamics, constraints, and different types of robots into nodes will be feasible. 
% Lastly, incorporating the naive path of a conflict zone into \textit{eta} edge features. The current representation only contains the naive duration of which a robot is inside a conflict zone. However, this neglects the scenario of two robots going in the same direction and never entering a conflict. Therefore, incorporating this information on the order of steps performed inside a conflict zone makes a more accurate conflict prediction possible.
Lastly, since the proposed method does not take into account the path to traverse a conflict zone, but only the duration, we will incorporate the path as a grid feature attribute in \textit{eta} edges in the future.


==> old_icra/experiments.tex <==

% \begin{table*}[b!]
% \centering
% \rowcolors{3}{}{white}
% \caption{Comparison of the model and prediction method.}
% \label{table:comparison}
% \resizebox{\textwidth}{!}{\begin{tabular}{| c | c |c c c|c c c|c c c|c c c|}
% \hline
% \multicolumn{2}{|c|}{Training settings} & \multicolumn{12}{c|}{Test environments with: } \\
% \hline
% \multirow{2}{*}{Methods}  & \multirow{2}{*}{Trained with}
% & \multicolumn{3}{c|}{250 robots}
% & \multicolumn{3}{c|}{500 robots} 
% % & \multicolumn{3}{c|}{750 robots} 
% & \multicolumn{3}{c|}{1000 robots}
% & \multicolumn{3}{c|}{Average} \\ %\cline{3-18}
%                                 &
%                                 &  RMSE & MAPE[\%] & MAE 
%                                 &  RMSE & MAPE[\%] & MAE 
%                                 &  RMSE & MAPE[\%] & MAE 
%                                 % &  RMSE[m] & MAPE[\%] & MAE[rad]
%                                 &  RMSE & MAPE[\%] & MAE\\
% \hline\hline
% \multirow{1}{*}{Naive ($A^*$)} 
%                                 &        
%                                 & 8.06 & 8.36 & 3.59 
%                                 & 13.45 & 12.79 & 6.80 
%                                 & 42.29 & 26.08 & 24.83
%                                 % & NaN & NaN & NaN 
%                                 & 21.27 & 15.74 & 11.74\\
% \hline\hline
% \rowcolor{lightgray}\cellcolor{white}               
%                                 & \cellcolor{white} 250 robots
%                                 & 7.18 & 4.59 & 3.19
%                                 & 12.26 & 8.75 & 5.99
%                                 & 38.36 & 21.15 & 21.81
%                                 % & NaN & NaN & NaN 
%                                 & 19.27 & 11.50 & 10.33 \\
                                
% \cellcolor{white}
%                                 & 500 robots
%                                 & 7.47 & 4.25 & 3.05
%                                 & 11.99 & 8.31 & 5.75
%                                 & 39.15 & 21.27 & 22.28
%                                 % & NaN & NaN & NaN 
%                                 & 19.54 & 11.28 & 10.36 \\
                                
%                                 % & 750 robots
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN 
%                                 % & NaN & NaN & NaN\\
                                
% \rowcolor{lightgray}\cellcolor{white}
% \multirow{-3}{*}{IMS}
%                                 & \cellcolor{white} 1000 robots 
%                                 & 7.36 & 4.53 & 3.15
%                                 & 11.70 & 8.31 & 5.66
%                                 & 37.79 & 20.46 & 21.30
%                                 % & NaN & NaN & NaN 
%                                 & 18.95 & 11.1 & 10.04\\
                                
% % \cellcolor{white}\multirow{-4}{*}{IMS}
% %                                 & 1-1000 robots 
% %                                 & NaN & NaN & NaN
% %                                 & NaN & NaN & NaN
% %                                 & NaN & NaN & NaN
% %                                 % & NaN & NaN & NaN 
% %                                 & NaN & NaN & NaN\\
% \hline \hline
% % \rowcolor{lightgray}
% \cellcolor{white}
%                                 & \cellcolor{white}250 robots
%                                 % RMSE,  MAPE,  MAE
%                                 & \textbf{6.14} & \textbf{3.72} & \textbf{2.52}
%                                 & 9.58 & 7.09 & 4.60
%                                 & 31.33 & 17.17 & 17.03
%                                 % & NaN & NaN & NaN 
%                                 & 15.68 & 9.33 & 8.05 \\
                                
% \rowcolor{lightgray}
% \cellcolor{white}               
%                                 & \cellcolor{white}500 robots
%                                 % RMSE,  MAPE,  MAE
%                                 & 6.38 & 3.78 & 2.60
%                                 & 9.17 & \textbf{6.91} & \textbf{4.44}
%                                 & 28.42 & 16.16 & 15.51
%                                 % & NaN & NaN & NaN 
%                                 & 14.66 & 8.95 & 7.52\\
                                
%                                 % & 750 robots
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN 
%                                 % & NaN & NaN & NaN\\
                                
% % \rowcolor{lightgray}
% \cellcolor{white} 
% \multirow{-3}{*}{DMS}              
%                                 &\cellcolor{white} 1000 robots 
%                                 % RMSE,  MAPE,  MAE
%                                 & 6.37 & 4.03 & 2.70
%                                 & \textbf{9.05} & 7.02 & 4.45
%                                 & \textbf{25.69} & \textbf{15.39} & \textbf{13.93}
%                                 % & NaN & NaN & NaN 
%                                 & \textbf{13.70} & \textbf{8.81} & \textbf{7.03}\\
                                
% % \cellcolor{white}\multirow{-4}{*}{DMS}
% %                                 & 1-1000 robots 
% %                                 & NaN & NaN & NaN
% %                                 & NaN & NaN & NaN
% %                                 & NaN & NaN & NaN
% %                                 % & NaN & NaN & NaN 
% %                                 & NaN & NaN & NaN\\
% \hline

% \end{tabular}}
% \end{table*}

\section{Experimental Setup}
\label{sec:experiments}
This section provides a concise description of the generated training and evaluation datasets, along with the error metrics used for evaluation and training parameters. The experiments focus on the prediction model and the accuracy as this is the varying factor of success. 
\subsection{Dataset}
\begin{figure}[t]
   \centering
   \includegraphics[width=0.49\textwidth]{images/experiments/map_example_v3.pdf}
   \caption{Examples of the randomly generated maps used for training and evaluation. The black pixels depict the occupied spaces, while the white pixels depict the free space.}
   \label{fig:map_examples}
\end{figure}

The GNN is trained on $5000$ unique generated warehouse environments of the size of a maximum $100\times 100$ meter. A few examples of generated maps are displayed in Fig. \ref{fig:map_examples}. The environments are populated with $N=\{250,500,1000\}$ robots, each with a corresponding goal point randomly distributed around the environment. In order to simulate up to $1000$ robot, time is recorded without considering acceleration, therefore moving a pixel will incur a fixed cost in time. The naive path is computed using Dijkstra for global planning and $A^*$ for local planning. For two reasons, the \ac{PIBT} and \ac{CBS} are not chosen as naive path planning methods. First, they modify the path of all robots and not just a single robot. Second, as the simulation is not considering acceleration, this is the perfect scenario for these methods, resulting in no conflicts. After performing the simulation, the actual arrival time is recorded and used as the label.

\subsection{Evaluation criteria}
The loss function used during training is the \ac{MAPE}. \ac{MAPE} computes the percentage between predicted values $\hat{y}$ and ground truth $y$: $MAPE = \frac{1}{m}\sum_{i=1}^{m}| \hat{y_i} - y_i | / y_i.$ It is the most popular metric for \ac{ETA} prediction tasks, as the percentage penalizes the relative distance error, making it robust against outliers compared to \ac{RMSE}, which is strongly penalizing the outliers with big errors.

\subsection{Training parameters}
The training and evaluation are conducted using an NVIDIA GeForce RTX 3090Ti GPU with 24GB VRAM. A high amount of VRAM is proven essential when training as the space required for computing the gradient of long temporal graphs is very high. However, the gradient is not computed during inference time, so a large amount of VRAM is no longer required. Due to the extensive use of VRAM, only a batch size of one is used during training. We use the Adam optimizer, while the learning rate $\gamma=0.001$ was scheduled to decay with $0.75$ every $8$th epoch. Each model has roughly trained 20 epochs, which with our hardware configuration would take $36$ to $48$ hours.
While training takes a long time to complete, the inference time is between $400$ to $700$ ms depending on the number of robots and the length of the paths.


% \subsection{Metrics}
% All comparison methods are evaluated by the metrics below:
% \begin{itemize}
%     \item \textbf{MAPE}: Mean Absolute Percentage Error computes the percentage between predicted values $\hat{y}$ and ground truth $y$: $MAPE = \frac{1}{m}\sum_{i=1}^{m}| \hat{y_i} - y_i | / y_i.$ MAPE is the most popular metric for the ETA tasks since the percentage is easier for people to conceptualize, and it is robust against outliers.
%     \item \textbf{MAE}: Mean Average Error calculates the absolute residual for each data point: $MAE = \frac{1}{m}\sum_{i=1}^{m}|\hat{y_i} - y_i|.$ A smaller MAE suggests the model is better at prediction.
%     \item \textbf{RMSE}: Root Mean Squared Error describes the spread of residuals: $RMSE = \sqrt{\frac{1}{m}\sum_{i=1}^{m}(\hat{y_i} - y_i)^2}.$
% \end{itemize}




==> old_icra/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% As part of industrial 4.0 and the need for more flexibility and efficiency, companies increasingly rely on \ac{AMR} to handle and distribute resources. Amazon is operating over $520.000$ robots across fulfillment and sort centers\cite{amazon-2022}, hereby running one of the largest \ac{AMR} systems. 
% The key component to successfully developing large-scale robotics systems is handling collision-free multi-agent path planning and controlling the flow of traffic. Intelligent transport systems and \ac{TrEPS} are widely used by transportation and logistic companies\cite{GOOGLE_ETA, traffic_pred}. However, the same technologies are rarely seen in indoor routing applications and even less in \ac{AMR} applications. Complications arise when introducing traditional \ac{TrEPS} in time-constrained \ac{AMR} routing applications.
The critical component of large-scale robotic systems is handling collision-free multi-agent path planning to control traffic flow systematically. Many logistic companies use intelligent transport and \ac{TrEPS}\cite{GOOGLE_ETA, traffic_pred}. However, these technologies are rarely used in indoor routing applications and even less in \acp{AMR} applications due to the complications when introducing traditional \ac{TrEPS} in time-constrained routing applications.
% Firstly, no road system is predefined, and mobile robots can move wherever there is free space. This increases the complexity of the planner as conflicts between two intersecting robots can occur anywhere along the trajectory.
The first challenge is that no road system is predefined, and \acp{AMR} can move wherever there is free space, which increases the planner complexity as conflicts between two intersecting robots can occur anywhere along the trajectory.
Secondly, traditional \ac{MAPF} is mainly motivated by path planning or motion planning for multi-robot systems \cite{PIBT, CBS}. However, the optimality or bounded suboptimality of \ac{MAPF} solutions does not necessarily entail their robustness. Robots often have imperfect plan execution capabilities and cannot synchronize their motions perfectly, resulting in frequent conflicts and time-expensive replanning \cite{ma2017overview}. 

% These problems are why we need \ac{TrEPS} to predict conflicts and adjust accordingly.
% Lastly, while allowing access to global information, \ac{AMR} is striving towards a decentralized system, allowing the robot only to change its own route. 

% In order to solve multi-objective path-planning problems faster, the incorporation of \ac{TrEPS} along with traditional path-planning algorithms is more commonly seen. \Ac{GNN} is commonly used in \ac{TrEPS} as they have demonstrated remarkable performance and generalize well to large-scale applications \cite{GOOGLE_ETA,traffic_pred, HEAT}. 

% This work focuses on developing a \ac{CAMAGP} for indoor multi-agent \ac{AMR} applications targeting time-constrained scenarios like logistics in airports or warehousing. What sets this work apart from the rest of the literature is the objective to not only want to find a route within a fixed time constraint but also to validate the effect caused by the route on the rest of the system by predicting \ac{ETA} for every agent in the system. 
This work focuses on developing a \ac{CAMAGP} for indoor multi-agent \ac{AMR} applications that target time-constrained scenarios, e.g., logistics in airports and warehouses. 
\ac{CAMAGP} is based on a two-layered framework. The first layer is a traditional path-planning algorithm for route suggestions which can be replaced by any appropriate path-planning algorithm. The second layer is the validation layer that validates the route suggested by the first layer and checks for time constraints. In order to validate a route, a graph is used to model spatio-temporal connectivity, and a \ac{GNN} is utilized for estimating traffic and predicting \ac{ETA}.
The objective of this research is not only to find a route within a fixed time constraint but also to validate the effect the route has on the rest of the system by predicting \ac{ETA} for each agent in the system. 
The performance of the proposed \ac{GNN} model is compared and contrasted with a naive method. 
In this work, the definition of \textit{naive} refers to paths that do not consider imperfect plan execution and the conflicts along the planned path. The naive time of arrival is the time it would take to perform such a naive path. 


\begin{figure}[t]
   \centering
   \includegraphics[width=0.49\textwidth]{images/introduction/drawing.pdf}
   \caption{Illustration of the multi-agent ETA prediction used in a warehouse environment. The values are the system-wide cost of taking the corresponding route, while the paths are relatively color-coded from the best (green) to the worst (red).}
   \label{fig:overview}
\end{figure}
The major contributions of this study are the followings:
\begin{itemize}
    \item A conflict-aware global planner is designed to optimize overall system flow while considering time constraints for all robots in industrial scenarios.
    \item A heterogeneous graph representation is proposed to model interaction between agents and potential bottle-neck areas occurring within the map. 
    %we propose an automatic bottle-neck detection and topological graph construction method from 2d occupancy grid maps.
    \item Finally, a novel \ac{GNN} architecture for multi-robot \ac{ETA} prediction in heterogeneous graphs is designed. 
\end{itemize}

The rest of this paper is organized as follows. 
Section \ref{sec:related_work} introduces the recent developments in \ac{TrEPS} and \ac{ETA} prediction. 
Section \ref{sec:methodology} provides the preliminaries for the problem formulation.
Section \ref{sec:experiments} presents the experiment setup followed by the \ac{CAMAGP} results in various grid world environments which are given in Section \ref{sec:results}. Finally, some conclusions are drawn from this study in Section \ref{sec:conclusion}.





==> old_icra/method.tex <==
\begin{figure*}[ht]
   \centering
   \includegraphics[width=0.98\textwidth]{images/Method/Network.pdf}
   \caption{Illustration of the proposed multi-agent ETA prediction framework. A simplified illustration of the three layers representing the indoor environment, as well as the connection between the layers, is shown on the left. The three layers consist of; a room-map segmenting the given grid map into artificial rooms, a static layer containing all nodes and edges with static information, and a dynamic layer containing the time-variant features of the graph. The proposed GNN architecture for multi-agent ETA prediction is also shown.}
   \label{fig:main}
\end{figure*}
\section{Methodology}
\label{sec:methodology}
% This section presents the four components of Map and graph representation, path-planning, eta-prediction, and constraint validation.

\subsection{Map and graph representation}
To predict multi-agent \ac{ETA} in an indoor environment, a room-map and spatio-temporal heterogeneous graph representation is proposed to capture the structure of the environment and the multiple route interaction.
The spatio-temporal heterogeneous graph is defined as follows:
\begin{equation}
G = (V, E, T_v, T_e, X_{v(t)}, X_{e(t)})  
\end{equation}
where $V$ is the set of nodes, $E$ is the set of edges, $T_v$ represents the node types belonging to the set $\{\text{robot}, \text{floor}\}$, $T_e$ represents the edge types belonging to the set $\{\text{eta},\text{association}\}$, $X_{v(t)}$ is the set of node-features at a given time $t$, and $X_{e(t)}$ is the set of edge-features at a given time $t$. 
The graph can further be deconstructed into two layers. 
A static layer containing nodes and edges with static features, and a dynamic layer containing nodes and edges with temporal features.
The objective of the room-map is to segment a grid-map into rooms and locate all passages connecting the rooms. 
The room-map is used to construct the static layer of the spatio-temporal heterogeneous graph and for route suggestions which will be described in Section \ref{PP}.
The three layers, room-map, static layer, and dynamic layer, and their interconnections are presented in Fig. \ref{fig:main}.
\medbreak
1) The proposed method expects a 2D topological grid-map of the environment containing static information about walls, rags, and non-parsing zones to construct the room-map.
The given grid-map is transformed into a homogeneous graph $G_{room}(V, E, X_v, X_e)$ where every corner is a node $v_i \in V$ and the node attribute $x_{v_i} \in X_v$ contains whether it is a concave or a convex corner. 
An edge $e_j \in E$ is either a solid surface like walls or a passage between two rooms. The corresponding attribute $x_{e_j} \in X_e$ is a one-hot encoding of whether it is a passage.
% Every surface is an edge , and its corresponding attribute $x_{e_j} \in X_e$ is whether it is a passage between rooms.
In order to construct passage edges, a ray-tracing is performed from every convex corner to the nearest neighboring static element.
If the ray-tracing hits an edge, the edge is split into two edges, and a node $v_{hit}$ is added in between.
A passage edge is constructed from the convex corner node $v_{start}$ to $v_{hit}$.

To divide the grid-map into rooms, a loop search is performed on the graph starting from every passage edge. 
The area bounded by the two shortest loops connected to each passage edge is defined as a room.
The rooms are then evaluated accordingly to their size and shape and merged with a neighboring room if they do not meet certain requirements.
These requirements are: no room is made up of less than four nodes, and the area of the room must be bigger than a threshold $A$, which is defined accordingly to the size of the map.
The last requirement is to merge small doorways, which are usually a group of four concave nodes close to each other. 

It is important to note that while these areas are defined as rooms, they do not necessarily fit the common definition of a room.
Instead, these map rooms are enclosed spaces surrounded by solid objects and passages, where the passages describe potential bottlenecks within the map.
An actual room can contain multiple of these map rooms located by this method. 

\medbreak
2) The static layer comprises all nodes and edges whose attributes are static and, therefore, will not change over time.
The nodes contained in this layer are of type \textit{floor}.
To construct \textit{floor} nodes, first the room-map is split into $N\times N$ patches.
A \textit{floor} node is constructed if any room tile occurs within a patch.
The feature of \textit{floor} nodes is the $N\times N$ patch.
A special case is if a solid line separates the patch.
Multiple \textit{floor} nodes are stacked, each representing a side of the patch, as the traffic on one side does not directly affect the other.
These stacked nodes are represented as multi-colored nodes in Fig. \ref{fig:main}.
The edges contained in the static layer are of type \textit{association}.
An association edge contains no features but represents a spatial link between two adjacent nodes or a self-loop.
An association edge is constructed when a direct path between two adjacent nodes can be established.

\medbreak
3) The dynamic layer contains all the nodes and edges with temporal features.
The nodes contained in this layer are of type \textit{robot} and the temporal feature of the node is the robot's priority.
The priority is computed based on the buffer time of each robot. 
\begin{equation}
\textit{priority}=(t_{current} + t_{path}) - t_{constraint}
\end{equation}
where $t_{current}$ is the current time, $t_{path}$ is the naive time of arrival and $t_{constraint}$ is the latest time of arrival.
This formulation can lead to deadlock if two robots are equal in priority.
Therefore the priority is rounded to the nearest integer and padded with the internal id as decimals to make the priority unique.
The edges in the dynamic layer are of type \textit{eta}.
\textit{Eta} edges are constructed from a \textit{robot} node to all \textit{floor} nodes passed in the corresponding path-plan of the robot.
The temporal features of \textit{eta} edges are the naive duration spent in \textit{floor} node, naive arrival time, and timestamp of the edge.
The timestamp portrays the order in which the \ac{GNN} processes the edges.

Lastly, all nodes contain a self-loop edge containing no features. The loop ensures the node's own features are combined with the neighboring features during the message passing layers. 

\subsection{Path-planner}
\label{PP}
An essential component in the proposed architecture is path-planning since a well-planned path can minimize the number of conflicts along the path. 
Traditional \ac{PIBT}\cite{PIBT} and \ac{CBS}\cite{CBS} calculates a conflict-free arrangement of paths for multi-agent systems.
However, they assume a constant cost in time for every movement, hereby not accounting for model parameters like acceleration and varying velocities.
As a result, the suggested paths can quickly become unsynchronized, leading to numerous conflicts.
The proposed framework can use any path-planning method since conflicts are accounted for during \ac{ETA} prediction.
The naive path planner chosen for the simulation is $A^*$\cite{a-star} because it does not account for any conflict.
Conflicts are solved online in the local planner using a priority-based system.
The robot with the highest priority keeps following its path while the others have to adapt their path.
Each robot declares the following five moves in a local area, and a local replanning is done to accommodate these intents based on priority.

A global graph is constructed from the room-map in order to generate route suggestions.
Each node in the graph represents a passage between rooms, while each edge connects all passages within the corresponding rooms.
The edge attributes are the distance between the passages calculated by a local planner.
A start node is added by locating the robot using the room-map and is connected to all associated passages within the found room.
The same procedure is done for the goal position.
Dijkstra \cite{dijkstra} is performed on the graph to determine the shortest route from the start to the goal.
In order to produce new paths in successive generations, the cost of the used edges is multiplied by $1.2$ after each iteration.
\medbreak
The path-planning module suggests plausible routes to the destination based solely on distance and the room-map layout.
Therefore ignoring the interaction of other agents in the system.
To validate the path's cost relative to the entire system, we have developed a \ac{GNN} architecture for multi-agent \ac{ETA} prediction for the entire system.

\subsection{Model architecture}
The architecture of the \ac{GNN} model is created accordingly to the encode-process-decode format illustrated in Fig. \ref{fig:main}. 
First, each node and edge in the heterogeneous graph is sent to the encoding layer.
An encoder is trained for each type of node and edge in the graph to extract specific type features into a $64$-dimensional feature vector.
The encoded nodes and edges are combined into the heterogeneous graph and passed to the attentive communication layers for message passing.

In the message passing module, we utilize the \ac{HEAT} operator\cite{HEAT}.
This operator enhances the \ac{GAT} \cite{GAT} by incorporating type-specific transformations of nodes and edges features during message passing. 
Similar to \ac{GAT}, \ac{HEAT} allows running several independent attention heads to stabilize the self-attention mechanism.
The features from each attention head are concatenated as the updated output feature.
The output of the \ac{HEAT} operator is the updated node features from the neighborhood of $K=1$ and $H=3$ number of attention heads concatenated.
The updated node features are passed to the edge updater module along with the encoded \textit{eta} edges.
In the edge updater module, the \textit{eta} edges are concatenated with the corresponding nodes and sent through a linear layer.

The decoder receives the \textit{eta} edges with timestamp $T$ and converts the eta feature vectors to \ac{ETA} predictions.
In the case of \ac{DMS}, the naive time of arrival of all \textit{eta} edges in the dynamic layer is updated based on the \ac{ETA} prediction to reflect the new predicted state of all robots. 
In the case of \ac{IMS}, the actual arrival time is used instead of the \ac{ETA} prediction. 
% Based on either the \ac{ETA} prediction in case of \ac{DMS} or the actual arrival time in case of \ac{IMS}, the naive time of arrival of all \textit{eta} edges in the dynamic layer is updated to reflect the new state of all robots.
As this is a recurrent process, this is repeated for $T=T+1$ until all \textit{eta} edges have been decoded.

\subsection{Validating time-constraints and path selection}
\label{cha:methodlogy}
There are numerous ways to validate a time constraint path, but choosing the optimal method relies heavily on the application at hand.
The proposed method rejects a path if one or more time constraints are not met.
In order to select the optimal valid path, the following cost is proposed: 
\begin{equation}
cost=\sum_{i=1}^{N}{\Bigl(\max{(\textit{TC})} - (\textit{TC}_{i} - \text{eta}_i)\Bigr)^2}  
\end{equation}
where \textit{TC} is the set of all the time constraints, \textit{eta} is the set of predicted \ac{ETA} for all $N$ robots.
The cost is constructed to maximize the buffer time between the constraint time and the predicted arrival time while penalizing the shorter buffer times and allowing more slack on the larger buffer times. 

==> old_icra/related_work.tex <==
\section{Related work}
\label{sec:related_work}
% \noindent Plan for this section
% \begin{enumerate}
%     \item Traditional methods
%     \item state of the art in ETA pred
%     \item state of the art in multi-agent prediction
% \end{enumerate}
 % This section introduces the foundation of \ac{MAPF}, \ac{GNN}, and \ac{STSF} to understand further the design choices of \ac{CAMAGP}.
\subsection{Traditional \ac{MAPF} solutions}
% While the proposed work does not directly solve the \ac{MAPF} problem, it is tightly correlated. Its primary objective is to validate the discovered route by assuming imperfect plan execution and forecasting conflicts along the route. 
 
State-of-the-art \ac{MAPF} methods can calculate collision-free paths for hundreds of agents with sub-optimal guarantees in reasonable amount of computation time\cite{PIBT, push_and_swap}. However, agents frequently have imperfect plan execution capabilities and cannot perfectly synchronize their motions, leading to frequent and time-consuming replanning. A post-processing framework is proposed in \cite{honig2016multi}, using a simple temporal graph to establish a plan-execution scheduler that guarantees safe spacing between robots.
% The work of \cite{honig2016multi} proposes a post-processing framework using a simple temporal graph to establish a plan-execution scheduler that guarantees safe spacing between robots.
The framework exploits the slack in time-constraints to absorb imperfect plan executions and prevent time-intensive replanning.

\subsection{Spatio-temporal graph neural networks}
A Spatio-temporal graph is a combination of spatio representing space or structural information and temporal representing time-varying information. 
Accordingly, if any system consists of a structural relationship between space and time, it can be represented as a spatio-temporal graph. These graphs can be used to design a neural network capable of handling static structures and time-varying characteristics. 
% We can define a spatio-temporal graph as a function of static structure and time-varying features:
% $$G = (V, E, X_{v(t)}, X_{e(t)})$$  
% where $G$ represents the graph, $V$ is the set of nodes, $E$ is the set of edges, $X_{v(t)}$ is the set of node-features at a given time $t$, and $X_{e(t)}$ is the set of edge-features at a given time $t$.

To work with spatio-temporal graphs, we must process a sequence of graph data to build a spatio-temporal embedding that may be used for regression, classification, clustering, or correlation prediction\cite{malla2021social}. The spatial block can be any conventional GNN \cite{battaglia2018relational}, while the temporal block can be any approach for learning over sequences of data, such as temporal convolution\cite{temporal-conv, temporal-conv-2} or temporal attention\cite{temporal-attention}. 
Various spatio-temporal \acp{GNN}  conform to the encoding-processing-decoding paradigm\cite{GOOGLE_ETA,battaglia2018relational, keisler2022forecasting}. This paradigm enables us to accommodate the iterative nature of \ac{STSF} and pathfinding algorithms. 
Improving these alignments has been shown to improve \acp{GNN} generalization to a more diverse distribution of graphs\cite{velivckovic2019neural}.
% 

\subsection{\ac{ETA} prediction and spatio-temporal sequence forecasting}
\label{sec:IMS-vs-DMS}
% Generally, \ac{ETA} predictions fall into the category of the \ac{STSF} problem.
The \ac{STSF} problem aims to predict a sequence of length $L$ into the future based on past observations and auxiliary data. The general learning strategies for multi-step forecasting fall into two major categories: \ac{IMS} estimation and \ac{DMS} estimation\cite{forecast_survey}. The \ac{IMS} strategy trains a one-step-ahead forecasting model and iteratively feeds the generated samples to the one-step-ahead forecaster to produce a multi-step-ahead forecast.
There are two main benefits of the \ac{IMS} strategy:
The one-step-ahead forecaster is simple to train because it only needs to consider the one-step-ahead forecasting error. It can generate predictions of any length by recursively applying the basic forecaster. The work of \cite{DCRNN} demonstrates how accounting for graph structure significantly reduces forecasting error across multiple horizons.
% Improving previous work, \cite{Gman} proposes the graph multi-attention network, a transform attention mechanism to transform the historical traffic features into future representations. This attention mechanism models direct relationships between historical and future time steps to alleviate the problem of error propagation.
% This design of spatial GNN combined with temporal component has yielded several subsequent proposals; STGCN\cite{STGCN}, GaAN\cite{GaAN}, ST-GRAT\cite{STGRAT}, and GMAN\cite{Gman}.
However, there is a disparity between the training and testing phase in \ac{IMS}.
In the training phase, the $L$th-step prediction is generated using the ground truths of the previous $L - 1$ steps. Though, during the testing phase, the model is provided with its previous prediction of the $L - 1$ steps rather than ground truths. This disparity makes the model susceptible to accumulating forecasting errors \cite{bengio2015scheduled}.

The primary objective of \ac{DMS} is to circumvent the accumulated error issue in \ac{IMS} by directly minimizing the long-term prediction error. Rather than training a single model, \ac{DMS} trains a distinct model $m_h$ for each forecasting horizon h. Therefore, the \ac{DMS} approach can support up to $L$ internal models. In order to separate the model size from the number of forecasting steps $L$, we can also construct $m_h$ by recursively applying the one-step-ahead forecaster $m_1$ in order to compute the multi-step-ahead forecasting error. It is worth noting that a multi-step-ahead forecasting error differs from a one-step-ahead forecasting error. Multi-step-ahead forecasting error accumulates the error during the sequence, while one-step-ahead forecasting error only minimizes for one step.
% This recursive \ac{DMS} method is widely adopted in deep learning-based methods including, Google maps\cite{GOOGLE_ETA}, Stg2seq\cite{Stg2seq}, Graph WaveNet\cite{wavenet}, and StemGNN\cite{StemGNN}.
Using \ac{DMS} does not come without cost\cite{chevillon2007direct}. \ac{DMS} is more computationally expensive than \ac{IMS}. For multi-model DMS, $L$ models need to be stored and trained, while recursive \ac{DMS} needs to apply $m_1$ for $\mathcal{O}(L)$ steps. Both cases require a large amount of memory storage or longer training time than solving the \ac{IMS} method. On the other hand, the \ac{IMS} training process is easily parallelizable since each forecasting horizon can be trained independently\cite{Goodfellow-et-al-2016}.

% Papers spatial–temporal graph neural network, GOOGLE_ETA,
In\cite{GOOGLE_ETA}, a homogeneous spatio-temporal \ac{GNN} method for predicting \ac{ETA} is proposed. While the main architecture consists of basic \ac{GNN} building blocks, they propose utilizing a combination of the recursive \ac{DMS} and multi-model \ac{DMS} to improve long horizon predictions. 
% Five models are trained using the recurrent \ac{DMS} for predicting $0$, $10$, $20$, $30$, and $60$ minutes into the futures. The model predicts the time it takes to traverse each node in the system during these five timeslots.
In \cite{huang2022dueta}, a focus on modeling traffic congestion propagation into a congestion-sensitive graph structure is proposed.
% Specifically, instead of directly using the road network as a graph, a congestion-sensitive graph based on the correlations of traffic patterns is introduced.
% In addition, a route-aware graph transformer layer is proposed to directly learn the road segment's long-distance correlations. 
In addition, a route-aware graph transformer layer is proposed enabling \acp{GNN} to capture the interactions between any road segments that are spatially distant but highly correlated with traffic conditions.
A novel heterogeneous graph structure is proposed in \cite{hong2020heteta}, which models both road features and historical data as heterogeneous information. It introduces edge features containing structural information on the relationship between nodes. In addition, three components are introduced to model temporal information from recent periods, daily periods, and weekly periods respectively. Each component comprises temporal convolutions and graph convolutions to learn representations of the spatio temporal heterogeneous information. 

While all the above-mentioned methods generate excellent results, they focus mainly on the features of the road and consider only a single vehicle traversing the graph. None of the models consider other types of vehicles driving in the environment or how the traffic is influenced due to the driver choosing the route. As a result, such models are not easily converted into multi-vehicle solutions.



% you should make comments and comparisons with these papers. One by one, please tell us what they have done and why it is good or bad. What is missing? and what contributions are made after this paper?

%Generally speaking, DMS is preferred for short-term prediction, where the dimensionality of data is very large, and only short-term predictions are required [5], [6]. IMS is preferred for long-term forecasts where the forecasting horizons are long, which are generally above 12 [4], [13] and can be as long as 100 [14].

% \textcolor{red}{Google maps example}
% When looking into how \ac{GNN} \cite{GOOGLE_ETA}



% Mapper
% Graph Neural Networks for Decentralized Multi-Robot Path Planning

==> old_icra/results.tex <==
\begin{table*}[!ht]
\centering
\rowcolors{3}{}{white}
\caption{Comparison of the model and prediction method.}
\label{table:comparison}
\resizebox{\textwidth}{!}{\begin{tabular}{| c | c |c c c|c c c|c c c|c c c|}
\hline
\multicolumn{2}{|c|}{Training settings} & \multicolumn{12}{c|}{Test environments with: } \\
\hline
\multirow{2}{*}{Methods}  & \multirow{2}{*}{Trained with}
& \multicolumn{3}{c|}{250 robots}
& \multicolumn{3}{c|}{500 robots} 
% & \multicolumn{3}{c|}{750 robots} 
& \multicolumn{3}{c|}{1000 robots}
& \multicolumn{3}{c|}{Average} \\ %\cline{3-18}
                                &
                                &  RMSE & MAPE[\%] & MAE 
                                &  RMSE & MAPE[\%] & MAE 
                                &  RMSE & MAPE[\%] & MAE 
                                % &  RMSE[m] & MAPE[\%] & MAE[rad]
                                &  RMSE & MAPE[\%] & MAE\\
\hline\hline
\multirow{1}{*}{Naive ($A^*$)} 
                                &        
                                & 8.06 & 8.36 & 3.59 
                                & 13.45 & 12.79 & 6.80 
                                & 42.29 & 26.08 & 24.83
                                % & NaN & NaN & NaN 
                                & 21.27 & 15.74 & 11.74\\
\hline\hline
\rowcolor{lightgray}\cellcolor{white}               
                                & \cellcolor{white} 250 robots
                                & 7.18 & 4.59 & 3.19
                                & 12.26 & 8.75 & 5.99
                                & 38.36 & 21.15 & 21.81
                                % & NaN & NaN & NaN 
                                & 19.27 & 11.50 & 10.33 \\
                                
\cellcolor{white}
                                & 500 robots
                                & 7.47 & 4.25 & 3.05
                                & 11.99 & 8.31 & 5.75
                                & 39.15 & 21.27 & 22.28
                                % & NaN & NaN & NaN 
                                & 19.54 & 11.28 & 10.36 \\
                                
                                % & 750 robots
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN 
                                % & NaN & NaN & NaN\\
                                
\rowcolor{lightgray}\cellcolor{white}
\multirow{-3}{*}{IMS}
                                & \cellcolor{white} 1000 robots 
                                & 7.36 & 4.53 & 3.15
                                & 11.70 & 8.31 & 5.66
                                & 37.79 & 20.46 & 21.30
                                % & NaN & NaN & NaN 
                                & 18.95 & 11.1 & 10.04\\
                                
% \cellcolor{white}\multirow{-4}{*}{IMS}
%                                 & 1-1000 robots 
%                                 & NaN & NaN & NaN
%                                 & NaN & NaN & NaN
%                                 & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN 
%                                 & NaN & NaN & NaN\\
\hline \hline
% \rowcolor{lightgray}
\cellcolor{white}
                                & \cellcolor{white}250 robots
                                % RMSE,  MAPE,  MAE
                                & \textbf{6.14} & \textbf{3.72} & \textbf{2.52}
                                & 9.58 & 7.09 & 4.60
                                & 31.33 & 17.17 & 17.03
                                % & NaN & NaN & NaN 
                                & 15.68 & 9.33 & 8.05 \\
                                
\rowcolor{lightgray}
\cellcolor{white}               
                                & \cellcolor{white}500 robots
                                % RMSE,  MAPE,  MAE
                                & 6.38 & 3.78 & 2.60
                                & 9.17 & \textbf{6.91} & \textbf{4.44}
                                & 28.42 & 16.16 & 15.51
                                % & NaN & NaN & NaN 
                                & 14.66 & 8.95 & 7.52\\
                                
                                % & 750 robots
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN
                                % & NaN & NaN & NaN 
                                % & NaN & NaN & NaN\\
                                
% \rowcolor{lightgray}
\cellcolor{white} 
\multirow{-3}{*}{DMS}              
                                &\cellcolor{white} 1000 robots 
                                % RMSE,  MAPE,  MAE
                                & 6.37 & 4.03 & 2.70
                                & \textbf{9.05} & 7.02 & 4.45
                                & \textbf{25.69} & \textbf{15.39} & \textbf{13.93}
                                % & NaN & NaN & NaN 
                                & \textbf{13.70} & \textbf{8.81} & \textbf{7.03}\\
                                
% \cellcolor{white}\multirow{-4}{*}{DMS}
%                                 & 1-1000 robots 
%                                 & NaN & NaN & NaN
%                                 & NaN & NaN & NaN
%                                 & NaN & NaN & NaN
%                                 % & NaN & NaN & NaN 
%                                 & NaN & NaN & NaN\\
\hline

\end{tabular}}
\end{table*}

\section{Results}
\label{sec:results}
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{images/Results/final_250.png}
    \caption{The absolute errors are plotted over the path length for the three \ac{DMS} models on the 250 robot test dataset. The shaded areas are the standard deviation over and under the mean absolute error for each of the three models.}
    \label{fig:length-comparison}
\end{figure}
% \begin{enumerate}
    % \item (Table) Compare DMS, IMS, and naive (All the loss functions) \ref{table:comparison}. 
    % \item (Graph) Prediction error over the length of the path.
    % \item (Graph) Prediction error over the number of robots.
% \end{enumerate}

\subsection{Method comparisons}
The first experiment compares the performance of the naive method, which does not use conflict-aware correction, the \ac{IMS} method, and the \ac{DMS} method. As shown in Table \ref{table:comparison}, using conflict-aware correction with either \ac{IMS} or \ac{DMS} significantly reduces error. Comparing the \ac{IMS} and \ac{DMS} methods, it is clear that the \ac{DMS} method is able to learn more from the training data. It is due to the accumulated error issue in \ac{IMS}, as explained in Section \ref{sec:IMS-vs-DMS}. There is a disparity between the training and testing phases, and as the density of robots rises and more conflict happens in the environment, the harder it is for the \ac{IMS} method to adapt to incorrect predictions. The best trained \ac{IMS} model improves the average \ac{MAPE} by 29.5$\%$ compared to the naive method, while the best \ac{DMS} model improves by 44$\%$. 

The second experiment demonstrates the relationship between prediction error and path length. As depicted in Fig. \ref{fig:length-comparison},  the prediction error generated by multi-step prediction methods accumulates in proportion to the path length. Since each prediction is based on the previous prediction, the standard deviation increases rapidly as the number of prediction iterations increases. Around the path length of $175$, the error curve plateau due to less number of robots moving, and hereby less conflict occurs. The standard deviation under the \ac{MAE} curve is smaller compared to above the curve. This depicts that the majority of the predictions lie beneath the \ac{MAE} curve with a smaller error. Contrarily, the standard deviation over the \ac{MAE} curve lies farther away, indicating that the model does not accurately predict a fewer number of paths, therefore generating big standard deviation errors.
% Since the three models have roughly the same curve structure, it seems the dataset could contain some outliers that all models are having trouble predicting.

\subsection{Generalization under different robot densities}
The third and final experiment demonstrates the generalization of the models in environments of varying densities. This is highly pertinent given that the number of robots can vary based on the season, demand, and business case. Therefore, for the industry to freely add or remove robots without retraining, the generalization of the model is of great importance.
As shown in Table \ref{table:comparison}, three different models trained on a dataset containing $250$, $500$, and $1000$ robots are compared at different densities. The results indicate that training in environments of high density generalizes well to environments of low density. This indicates that none of the models are overfitting to any density-specific features in the graph representation. 

The \ac{DMS} models trained with the same number of robots as in the test scenario generally perform slightly better, as depicted in bold in Table. \ref{table:comparison}. However, in the $500$ robot test environment, the $1000$ robot \ac{DMS} model outperforms the $500$ robot \ac{DMS} model in terms of \ac{RMSE}. As more conflicts are happening in higher density environments, the $1000$ robot \ac{DMS} model is generally trained on paths much longer compared to the $500$ robot \ac{DMS} model. As a result, since \ac{RMSE} is sensitive to longer paths as they are accumulating more errors, as shown in experiment two, the $1000$ robot \ac{DMS} is better suited for outliers occurring within the $500$ robot test dataset.
The last column of Table \ref{table:comparison} shows average results in all the test environments. The \ac{DMS} model trained on $1000$ robots has proven to be the most generalized model.

==> old_iros/abstract.tex <==
% This study proposes a conflict-aware multi-agent estimate time of arrival (CAMAETA) framework for predicting the time of arrival of all agents in environments without any predefined road infrastructure. 
% The framework comprises of three layers: a traditional path planning algorithm for suggesting paths, a path evaluation layer for predicting multi-agent estimate time of arrival times for all agents, and lastly a cost layer for computing the best overall path suggested by the first layer. The novelty of the framework lies in the heterogeneous map representation along with a novel heterogeneous graph neural network architecture for multi-agent arrival time estimation. Unlike existing methods that rely on structured road infrastructure and historical data to predict time of arrival, the proposed framework utilizes total path length and basic structural features, resulting in improved generalization capabilities. To the best of our knowledge, this is the first attempt to predict multi-agent arrival times without structured road infrastructure. The results of extensive simulations demonstrate the accuracy and effectiveness of the proposed method, and show improvements in mean average percentage error of 29.5\% and 44\% when compared to a naive method that does not consider conflicts.
This study presents the conflict-aware multi-agent estimated time of arrival (CAMETA) framework, a novel approach for predicting the arrival times of multiple agents in unstructured environments without predefined road infrastructure. The CAMETA framework consists of three components: a path planning layer generating potential path suggestions, a path evaluation layer predicting the arrival times for all agents based on the paths, and lastly, a path selection layer that calculates the accumulated cost and selects the best path. The novelty of the CAMETA framework lies in the heterogeneous map representation and the heterogeneous graph neural network architecture. As a result of the proposed novel structure, CAMETA improves the generalization capability compared to the state-of-the-art methods that rely on structured road infrastructure and historical data. The simulation results demonstrate the efficiency and efficacy of the multi-agent ETA prediction layer, with a mean average percentage error improvement of 29.5\% and 44\% when compared to a traditional path planning method ($A^*$) which does not consider conflicts. The performance of the CAMETA framework shows significant improvements in terms of robustness to noise and conflicts as well as determining proficient routes compared to state-of-the-art multi-agent path planners.



%The framework consists of a novel heterogeneous map representation, traditional path planning algorithm, and novel heterogeneous graph neural network architecture for multi-agent arrival time estimation. Instead of relying on the structured road infrastructure and historical data to predict the time of arrival, the proposed framework benefits from the total path length and basic spatial features, which has better generalization capability. To the best of our knowledge, this work is the first attempt to predict multi-agent arrival times without any structured road infrastructure. The extensive simulation results illustrate the accuracy and efficacy of the proposed method, demonstrating its feasibility and effectiveness. Compared to a naive method that does not consider conflict, the best-trained iterative multi-step model improves the overall mean average percentage error by 29.5\%, while the best direct multi-step model improves by 44\%.



% %As the popularity of autonomous mobile robot applications is rising in the industry, conflict-aware multi-agent path planning becomes essential for a smooth and efficient operation of autonomous robots in highly dynamic environments.
% This study proposes a framework for a Conflict Aware Multi-Agent Global Planner (CAMAGP), which combines novel heterogeneous map representation, traditional path-planning algorithms, and a novel heterogeneous graph neural network architecture for multi-agent arrival time estimation. 
% % The proposed framework relies not on historical data but on naive path distance along with the structural features of the path. As a result, the framework does not depend on structured road infrastructure in order to predict the arrival time.
% Contrary to other methods, which rely on structured road infrastructure and historical data to predict the time of arrival, the proposed framework only relies on the total path length and basic structural features, thus making it more general in its application.
% % Since the proposed framework does not rely on historical data but uses naive path distance and structural features of the path, the framework does not depend on a structured road infrastructure to predict the arrival time.
% To the best of our knowledge, this work is the first attempt to predict multi-agent arrival times without any structured road infrastructure. 
% Compared to a naive method that does not consider conflict, the best trained iterative multi-step model improves the overall mean average percentage error by 29.5\%, while the best direct multi-step model improves by 44\%.
% The results illustrate the accuracy and efficacy of the proposed method, demonstrating its feasibility and effectiveness.

% % NOTE:
% % Since the first sentence of the paragraph will be deleted, you will have some extra space in your abstract. How about keeping this sentence but adding a few details to your results by adding one more sentence before this sentence? you can write one or two significant discussions for your results. For example: 
% % "The best trained IMS model improves the average MAPE by 29.5% compared to the naive method, while the best DMS model improves by 44%"


==> old_iros/conclusion.tex <==

\section{Conclusion and future work}
\label{sec:conclusion}
% In this work, we conduct pioneering research by developing a framework for predicting conflicts and estimating the time of arrival in a multi-agent environment. We formulate our problem as a spatio-temporal graph focusing on edge prediction. This allows for the estimated time of arrival prediction of all robots simultaneously, which previous work has not been able to accomplish. While this is the first study in the field on systemwide estimated time of arrival, it has been demonstrated to increase the accuracy of the predicted time of arrival. As a result, the overall framework's capacity to accurately evaluate the cost of each route improves. 

% In future work, a couple of features could be incorporated into the current framework. Firstly, incorporate robot acceleration to reflect the real-world dynamics more accurately. Secondly, include multiple types of robots. As we are representing the problem as a heterogeneous graph, incorporating dynamics, constraints, and different types of robots into nodes is very feasible. 
% Lastly, incorporating the naive path of a conflict zone into \textit{eta} edge features. The current representation only contains the naive duration of which a robot is inside a conflict zone. However, this neglects the scenario of two robots going in the same direction and never entering a conflict. Therefore, incorporating this information on the order of steps performed inside a conflict zone makes a more accurate conflict prediction possible.

% As future work, we plan to incorporate a more accurate robot motion model as well as turn the simulation into continuous space in order to reflect real-world dynamics more accurately. We will also include multiple types of robots in the same environment. As we represent the problem as a heterogeneous graph, incorporating dynamics, constraints, and different types of robots into nodes will be feasible. 
% Lastly, since the proposed method does not take into account the path traversed inside a floor tile, but only the duration, we will incorporate the path as a grid feature attribute in \textit{eta} edges in the future.


In this work, we develop a framework to predict conflicts and \ac{ETA} in multi-agent environments. We formulate our problem as a spatio-temporal graph focusing on edge prediction. The proposed methodology allows \ac{ETA} prediction of all robots simultaneously, which was not possible by the previously published works. Through extensive simulation experiments, the proposed method demonstrates an increase in the accuracy of the predicted arrival time. 
% While this is the first study on the system-wide estimated time of arrival, we also 
It should be noted that our proposed framework does not solve the \ac{MAPF} problem as it does not provide collision-free paths for each agent. Instead, we employ the use of \ac{ETA} in order to minimize the number of conflicts that an online path-planning algorithm needs to resolve, resulting in a more resilient method that is better equipped to handle noise.

As future work, we aim to enhance the framework by incorporating a more sophisticated robot motion model and transitioning to a continuous space simulation to better reflect real-world dynamics. Additionally, we plan to extend the framework to include multiple types of robots in a heterogeneous graph representation, incorporating dynamics, constraints, and different types of robots as nodes. Furthermore, we will incorporate the path traversed within a floor tile as a feature attribute in the \textit{eta} edges.

==> old_iros/experiments.tex <==
\section{Experimental Setup}
\label{sec:experiments}
This section concisely describes of the generated training and evaluation datasets, along with the error metrics used for evaluation and training parameters. The first set of experiments focuses on evaluating the accuracy of the \ac{ETA} prediction model, as it is a critical factor for the success of the proposed framework. The second set of experiments compares the proposed framework with state-of-the-art offline planners to assess its overall performance.

\subsection{Simulation environment and noise}
The simulation scenario is based on a discrete grid world where each agent carries out a single action at each time step. The movement of the robots is modeled to operate at full velocity, and as such, the inclusion of noise in the simulation would not result in increased speed. On the contrary, the presence of noise would slow down the movement of the robots, causing them to force a wait action when the noise accumulates to a certain extent.
Offline path planners are evaluated in terms of their robustness to conflicts and imperfections in plan execution due to noise. The experiment is designed to assess the impact of varying levels of imperfect plan execution noise, which are set to the following degrees: $\{0\%, 0.00001\%, 0.0001\%, 0.001\%, 0.01\%\}$. These levels correspond to the probability of a forced wait action resulting from accumulated noise.

We develop the \ac{ETA} prediction module without taking into account the presence of noise in order to avoid any potential bias towards a pre-defined noise level. 
% Although it could be argued that noise could be considered a simplified motion model parameter, for the purpose of ensuring fairness in comparison with other planning methods, the decision was made not to include noise in the training process of the prediction module. 
However, during the evaluation of the overall framework, noise was introduced to all methods to conduct a more comprehensive analysis.

The experiments utilize the \ac{WHCA*} priority method as the online planner to resolve any conflicts that may arise during the simulation. This method was chosen for its simplicity, efficiency, and integration of priority selection into the algorithm.


\subsection{Estimate time of arrival prediction}
\subsubsection{Training data}
\begin{figure}[t]
   \centering
   \includegraphics[width=0.49\textwidth]{images/experiments/Maps-2.pdf}
   \caption{The figure illustrates several examples of the maps utilized in training the multi-agent \ac{ETA} prediction module (enclosed in red), and the map utilized for evaluating the overall performance of the system (enclosed in blue). The depiction of the black pixels indicates occupied spaces, while the white pixels signify unoccupied areas.}
   \label{fig:map_examples}
\end{figure}

The \ac{GNN} is trained on $5000$ unique generated warehouse environments of the size of a maximum $100\times 100$ meter. A few examples of generated maps are displayed in Fig. \ref{fig:map_examples}. The environments are populated with $N=\{250,500,1000\}$ robots, each with a corresponding goal point randomly distributed around the environment. 
%Different
The naive path is computed using the $A^*$ algorithm, which is used as initial input to the \ac{GNN} model. \ac{PIBT} and \ac{CBS} are not chosen as naive path planning methods for a couple of reasons. First, they modify the path of all robots and not just a single robot. Second, as the training simulation does not consider any noise or imperfect plan execution, this is the perfect scenario for these methods, resulting in no conflicts. After performing the simulation, the actual arrival time is recorded and used as the label.

\subsubsection{Evaluation criteria}
The loss function used during training is the \ac{MAPE}. \ac{MAPE} computes the percentage between predicted values $\hat{y}$ and ground truth $y$: $MAPE = \frac{1}{m}\sum_{i=1}^{m}| \hat{y_i} - y_i | / y_i.$ It is the most popular metric for \ac{ETA} prediction tasks, as the percentage penalizes the relative distance error, making it robust against outliers compared to \ac{RMSE}, which is strongly penalizing the outliers with big errors.

\subsubsection{Training parameters}
The training and evaluation are conducted using an NVIDIA GeForce RTX 3090Ti GPU with 24GB VRAM. A high amount of VRAM is proven essential when training as the space required for computing the gradient of long temporal graphs is very high. However, the gradient is not computed during inference time, so a large amount of VRAM is no longer required. Due to the extensive use of VRAM, only a batch size of one is used during training. We use the Adam optimizer, while the learning rate $\gamma=0.001$ was scheduled to decay with $0.75$ every $8$th epoch. Each model has roughly trained 20 epochs, which with our hardware configuration, would take $36$ to $48$ hours.
While training takes a long time to complete, the inference time is between $400$ to $700$ ms depending on the number of robots and the length of the paths.

\subsection{Evaluation of the offline path planners}
% In this experiment, the performance of offline path planners is evaluated in terms of their robustness to conflicts and imperfections in plan execution due to noise. The experiment is designed to assess the impact of varying levels of imperfect plan execution noise, which are set to the following degrees: $\{0\%, 0.00001\%, 0.0001\%, 0.001\%, 0.01\%\}$. These levels correspond to the probability of a forced wait action resulting from accumulated noise.
% Four different offline path planning methods will be compared for their robustness in the presence of conflicts and plan execution noise. The methods to be compared include: $A^*$, \ac{PIBT}, \ac{CBS}, and \ac{CAMETA}.

The proposed method \ac{CAMETA} is evaluated against other offline path planning methods, including $A^*$, \ac{PIBT}, and \ac{CBS} with respect to their robustness in the presence of conflicts and plan execution noise.
The $A^*$ is chosen as a method that does not take into account the presence of other agents or conflicts in the paths being planned. \ac{PIBT} is chosen as a suboptimal method that is designed to be computationally efficient and considers both all agents and conflicts. \ac{CBS} is chosen as an optimal method. Although less computationally efficient than \ac{PIBT} and cannot run in real-time, it is able to determine the optimal paths for all agents.
% Finally, \ac{CAMETA} is a conflict-aware approach, which aims to minimize conflicts by estimating the time required to resolve the whole path, including the conflict, rather than relying on paths that are conflict-free.

The environment chosen for the experiment is shown in Fig. \ref{fig:map_examples} enclosed in blue. The map features both open spaces as well as corridors and potential bottlenecks. Each experiment will be conducted with $500$ agents and repeated $100$ times with different seeds of noise to eliminate a method being unlucky with the noise. However, the starting position and destination of robots will remain the same across all methods and seeds. The average \textit{makespan}, which is the average time for all robots to finish, and the sum of costs are presented in the results section.

==> old_iros/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\begin{figure}[t]
   \centering
   \includegraphics[width=0.43\textwidth]{images/introduction/Framework_Structure_v3.pdf}
   \caption{The conflict-aware multi-agent planner framework is depicted in three layers. The first layer generates multiple path suggestions for a single agent. The second layer, enclosed in blue borders, produces estimated time of arrival predictions for all agents. Finally, the third layer computes the overall cost for each suggested path, using the information generated in the previous layer.}
   \label{fig:overview}
 
\end{figure}

% The critical component of large-scale robotic systems is handling collision-free multi-agent path planning to control traffic flow systematically. Many logistic companies use intelligent transport and \ac{TrEPS}\cite{GOOGLE_ETA, traffic_pred}. However, these technologies are rarely used in indoor routing applications and even less in \acp{AMR} applications due to the complications when introducing traditional \ac{TrEPS} in time-constrained routing applications.

% The first challenge is that no road system is predefined, and \acp{AMR} can move wherever there is free space, which increases the planner complexity as conflicts between two intersecting robots can occur anywhere along the trajectory.
% Secondly, traditional \ac{MAPF} is mainly motivated by path planning or motion planning for multi-robot systems \cite{PIBT, CBS}. However, the optimality or bounded suboptimality of \ac{MAPF} solutions does not necessarily entail their robustness. 


% These problems are why we need \ac{TrEPS} to predict conflicts and adjust accordingly.
% Lastly, while allowing access to global information, \ac{AMR} is striving towards a decentralized system, allowing the robot only to change its own route. 

% In order to solve multi-objective path-planning problems faster, the incorporation of \ac{TrEPS} along with traditional path-planning algorithms is more commonly seen. \Ac{GNN} is commonly used in \ac{TrEPS} as they have demonstrated remarkable performance and generalize well to large-scale applications \cite{GOOGLE_ETA,traffic_pred, HEAT}. 

\Ac{MAPF} is the problem of generating valid paths for multiple agents while avoiding conflicts. This problem is highly relevant in many real-world applications, such as logistics, transportation, and robotics, where multiple agents must operate in a shared environment. \ac{MAPF} is a challenging problem due to the need to find paths that avoid conflicts while minimizing the overall travel time for all agents. Many state-of-the-art \ac{MAPF} solvers \cite{CBS, PIBT, HCA*} employ various techniques to find a set of conflict-free paths on graphs representing the environment and the agents. However, a common limitation of these solvers is that they tend to generate tightly planned and coordinated paths. Therefore, the agents are expected to follow the exact path prescribed by the solver, which can lead to problems when applied to real-world systems with imperfect plan execution and uncertainties in the environment.

% In this work, we propose a \ac{CAMETA} for indoor multi-agent \ac{AMR} applications that operate in time-constrained scenarios. \ac{CAMETA} is a three-layered framework deployed on every agent. The layers consist of: a path planning layer producing route suggestions for the current agent, a multi-agent \ac{ETA} prediction layer forecasting \ac{ETA} prediction of all agents in the system given one of the suggested paths, and a cost validation layer minimize the overall travel time by reducing the total number of conflicts in the system. The proposed framework is illustrated in Fig. \ref{fig:overview}. In our problem definition, some agents need to arrive at their destination quicker than other agents in a system, e.g., logistics in airports and warehouses.


This work introduces a \ac{CAMETA} for indoor \ac{AMR} applications that operate in time-constrained scenarios. The proposed framework is a three-layered framework that is deployed on each agent. The layers consist of a path planning layer, which generates route suggestions for the deployed agent, a multi-agent \ac{ETA} prediction layer, which forecasts the \ac{ETA} of all agents in the system given one of the suggested paths, and a cost validation layer that minimizes the overall travel time by reducing the total number of conflicts in the system. In our problem definition, some agents are required to arrive at their destination quicker than others, which is a common scenario in logistics applications for airports and warehouses. The proposed framework is illustrated in Fig. \ref{fig:overview}.


% In systems with multiple moving agents, valid paths must be provided to ensure that agents reach their destinations smoothly without any conflicts, while minimizing excess travel time. This problem is embodied in \ac{MAPF}, which aims to find a set of conflict-free paths on graphs.
% Many state-of-the-art \ac{MAPF} solvers \cite{CBS, PIBT, HCA*} tents to produce paths that are too tightly planned and coordinated in order to optimize the objective of finding the shortest paths without taking into consideration imperfect plan execution or noise.  

% This work focuses on developing a \ac{CAMETA} for indoor multi-agent \ac{AMR} applications that target time-constrained scenarios. In our problem definition, some agents need to arrive at their destination quicker than other agents in a system, e.g., logistics in airports and warehouses. The overall framework is illustrated in Fig. \ref{fig:overview}.

% The proposed framework is based on a three-layered structure, as illustrated in Fig \ref{fig:overview}. The first layer comprises a traditional path-planning algorithm that proposes various route suggestions. 
% The second layer aims to evaluate the proposed routes by forecasting the \ac{ETA} for each agent. The objective of the layer is to anticipate the impact of the proposed path on the other agents within the system and to estimate the additional time added by these effects. To estimate the \ac{ETA} of all agents, this study employs a graph-based approach to model the spatio-temporal connectivity of the system. This graph is then provided to a recurrent \ac{GNN} model for prediction. 
% The third layer utilizes the \ac{ETA} to evaluate time-constraints and calculate the cost of each suggested route. The layer is not only used to find a route that is feasible within a fixed time constraint but it is also used to validate the impact of the chosen route on the rest of the system by utilizing the predicted \ac{ETA} for all agents. The first and last layers of the framework are designed to be modular and can be easily substituted with more application-specific methods. 

% In order to validate a route, a graph is used to model spatio-temporal connectivity, and a \ac{GNN} is utilized for estimating traffic and predicting \ac{ETA}.
% The objective of this research is not only to find a route within a fixed time constraint but also to validate the effect the route has on the rest of the system by predicting \ac{ETA} for each agent in the system. 

This work mainly focuses on the development of the multi-agent \ac{ETA} prediction layer and its effectiveness in forecasting the \ac{ETA} for each agent. To evaluate the multi-agent \ac{ETA} prediction layer and the proposed \ac{GNN} model, this study compares it to a naive method. In this context, the term \textit{"naive"} refers to paths, which does not consider the imperfect execution of plans and conflicts that may occur along the planned path. 
% The naive time of arrival is defined as the time it would take to complete such a naive path.
This comparison provides insight into the performance and accuracy gained by utilizing the \ac{GNN} model for predicting \ac{ETA} as opposed to ignoring the complexities such as imperfect execution and conflicts. Lastly, An experiment is conducted to demonstrate the proposed framework's overall performance compared to state-of-the-art methods \cite{CBS, PIBT}.

The contributions of this study are the followings:
\begin{itemize}
    \item A conflict-aware global planner is designed to optimize overall system flow while considering time constraints for all robots in industrial scenarios.
    \item A heterogeneous graph representation is proposed to model the interaction between agents and potential bottle-neck areas occurring within the map. 
    %we propose an automatic bottle-neck detection and topological graph construction method from 2d occupancy grid maps.
    \item Finally, a novel \ac{GNN} architecture for multi-robot \ac{ETA} prediction in heterogeneous graphs is designed. 
\end{itemize}

The rest of this paper is organized as follows. 
Section \ref{sec:related_work} reviews the recent developments in \ac{MAPF} and \ac{ETA} prediction. 
Section \ref{sec:methodology} provides the details of the proposed framework.
Section \ref{sec:experiments} presents the experiment setup followed by the results in various grid world environments in Section \ref{sec:results}. Finally, some conclusions are drawn from this study in Section \ref{sec:conclusion}.





==> old_iros/method.tex <==
\begin{figure*}[ht]
   \centering
   \includegraphics[width=0.98\textwidth]{images/Method/Network_no_room_map.pdf}
   \caption{Illustration of the proposed multi-agent \ac{ETA} prediction layer. A simplified illustration of the three layers representing the indoor environment, as well as the connection between the layers, is shown on the left. The three layers consist of: a 2D occupancy grid map of the environment, a static layer containing all nodes and edges with static information, and a dynamic layer containing the time-variant features of the graph. The proposed \ac{GNN} architecture for multi-agent \ac{ETA} prediction is also shown.}
   \label{fig:main}
\end{figure*}
\section{Methodology}
\label{sec:methodology}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% PATHPLANNING %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Path planning}
\label{PP}
The path planning layer is similar in design to the \ac{LRA*}\cite{LRA*}, where other agents in the system are not considered, and resolving conflicts is left to the online planner. This allows for a decentralized offline planning module, where each agent only needs to consider possible routes to its destination. While drastically improving scalability, it comes with the limitation of not being able to change the routes of other agents.
Essentially the consideration of other agents is first introduced in the second layer, where \ac{ETA} is computed for all agents.

The offline planner chosen for this framework is $A^*$\cite{a-star}, as it does not account for conflicts and can quickly compute different route suggestions. Conflicts are resolved online using the \ac{WHCA*} \cite{HCA*} algorithm with a priority-based system. The robot with the highest priority maintains its path while others adapt their paths. Each robot declares its next five moves in a local area, and local replanning is done based on priority. Agents require local communication and priority-based bidding to align the reservation of space.

The proposed framework can use any off-the-shelf path-planning methods since conflicts are accounted for during the \ac{ETA} prediction in the second layer. It is important to note that the \ac{GNN} is trained based on both the online and offline path planning algorithm and, therefore, still dependent on these. The \ac{GNN} model learns to model the interactions between these two planners, including how much the offline path-planning algorithm considers conflicts in its route suggestions and how effectively the online path-planning algorithm resolves conflicts.

\subsection{Multi-agent estimated time of arrival prediction} 
The multi-agent estimated time of arrival layer is the second layer of the system. The objective of the layer is to anticipate the impact of the proposed path on the other agents within the system and to estimate the additional time added by these effects. It takes as input the suggested routes from the first layer, as well as the planned paths of all other agents, and a 2D occupancy grid map of the environment in order to predict the \ac{ETA} for each agent. The layer is composed of two main steps: It reconstructs the data into a spatio-temporal heterogeneous graph representation and then passes the graph through a recurrent spatio-temporal \ac{GNN} model in order to make the \ac{ETA} predictions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% GRAPH REPRESENTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Graph representation}
% To predict multi-agent \ac{ETA} in an indoor environment, a spatio-temporal heterogeneous graph representation is proposed to capture the structure of the environment and the multiple route interaction.
To predict the \ac{ETA} of multiple agents in an indoor environment, a spatio-temporal heterogeneous graph representation is used to capture the environment's structure and the interactions between routes. The graph is divided into two layers: a static layer and a dynamic layer. The interaction between the layers is depicted in Fig. \ref{fig:main}.

The static layer of the graph only needs to be constructed once, as its features and connections remain unchanged. The static layer contains nodes of type \textit{floor} with static features of the environment, such as walls, restricted areas, and open spaces. The edges in the static layer are of type \textit{association} and represent the spatial links between nodes. The spatial characteristics of the environment are obtained from a 2D occupancy grid map, which is divided into $N\times N$ tiles. A node of type  \textit{floor} is constructed for each tile created from the given map, and the node features are the spatial information within the tile. In order to lower the number of floor nodes, all nodes containing only occupied space are removed. In the case of a solid line separating a tile, multiple \textit{floor} nodes are stacked to represent each side of the patch, as traffic on one side does not directly impact the other. These stacked nodes are depicted as multi-colored nodes in Fig. \ref{fig:main}. Association edges contain no features and are created when a direct path between two adjacent nodes or a self-loop is established.

The dynamic layer consists of nodes and edges with temporal features, where the features are subject to change or removal in the recurrent stages of the \ac{GNN} model. Nodes in this layer are of type \textit{robot}, and the temporal feature of each node is the robot's priority, computed based on the buffer time between the current time estimation and the constraint time of the robot task.  If two robots have equal priority, the priority is rounded to the nearest integer and appended with the robot's internal ID as decimals to make it unique to avoid deadlocks. Edges in the dynamic layer are of type \textit{eta} and are created from a \textit{robot} node to all \textit{floor} nodes in the robot's planned trajectory. All outgoing \textit{eta} edges from a \textit{robot} node represent the planned path for the corresponding robot. The temporal features of the \textit{eta} edges include the estimated duration at each \textit{floor} node, the estimated arrival time, and the timestamp of the edge. The timestamp reflects the order in which the \ac{GNN} processes the edges. All nodes contain a self-loop edge, which has no features, to ensure that the node's own features are combined with those of its neighbors during the message-passing phase.

Combining the dynamic and static layer, the spatio-temporal heterogeneous graph is defined as follows:
\begin{equation}
G = (V, E, T_v, T_e, X_{v(t)}, X_{e(t)})  
\end{equation}
where $V$ is the set of nodes, $E$ is the set of edges, $T_v$ represents the node types belonging to the set $\{\text{robot}, \text{floor}\}$, $T_e$ represents the edge types belonging to the set $\{\text{eta},\text{association}\}$, $X_{v(t)}$ is the set of node-features at a given time $t$, and $X_{e(t)}$ is the set of edge-features at a given time $t$. 
% The graph can be categorized into two layers; a static layer and a dynamic layer. 
% The static layer contains nodes and edges with static features of the environment, such as walls, restricted areas, and open spaces, while the dynamic layer consists of nodes and edges with temporal features that change over time, capturing the dynamic movement and interactions between agents. The interaction between the layers is depicted in Fig. \ref{fig:main}.

% \medbreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% STATIC LAYER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The static layer of the graph only needs to be constructed once, as its features and connections remain unchanged. The spatial characteristics of the environment are obtained from a 2D occupancy grid map, which is divided into $N\times N$ tiles. A node of type  \textit{floor} is constructed for each tile created from the given map, and the node features are the spatial information within the tile. In order to lower the number of floor nodes, all nodes containing only occupied space are removed. In the case of a solid line separating a tile, multiple \textit{floor} nodes are stacked to represent each side of the patch, as traffic on one side does not directly impact the other. These stacked nodes are depicted as multi-colored nodes in Fig. \ref{fig:main}. 
% The edges in the static layer are of type \textit{association} and serve to represent the spatial links between nodes. Association edges contain no features and are created when a direct path between two adjacent nodes or a self-loop is established.

% \medbreak
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% DYNAMIC LAYER %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The dynamic layer comprises nodes and edges with temporal features. The features of the nodes and edges in this layer are subject to change or removal in the recurrent stages of the \ac{GNN} model. The nodes in the dynamic layer are of type \textit{robot}, and the temporal feature of each node is the robot's priority which is computed based on the buffer time between the current time estimation and the constraint time of the robot task as follows.
% \begin{equation}
% \textit{priority} = (t_{current} + t_{path}) - t_{constraint}
% \end{equation}
% where $t_{current}$ is the current time, $t_{path}$ represents the estimated time of arrival, and $t_{constraint}$ is the latest time of arrival. If two robots have equal priority, the priority is rounded to the nearest integer and appended with the robot's internal ID as decimals to make it unique to avoid deadlocks. The edges in the dynamic layer are of type \textit{eta}. 
% These edges are created from a \textit{robot} node to all \textit{floor} nodes that are included in the robot's planned trajectory. Specifically, whenever a robot is planned to traverse a tile, an edge is created to the corresponding \textit{floor} node. The temporal features of the \textit{eta} edges include the estimated duration at each \textit{floor} node, the estimated arrival time, and the timestamp of the edge. The timestamp reflects the order in which the \ac{GNN} processes the edges. Additionally, all nodes contain a self-loop edge, which has no features. The loop ensures that the node's own features are combined with those of its neighbors during the message-passing phase.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% MODEL ARCHITECTURE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Model architecture}
The architecture of the \ac{GNN} model is created accordingly to the encode-process-decode format illustrated in Fig. \ref{fig:main}. 
First, each node and edge in the heterogeneous graph is sent to the encoding layer.
An encoder is trained for each type of node and edge in the graph to extract specific type features into a $64$-dimensional feature vector.
The encoded nodes and edges are combined into the heterogeneous graph and passed to the attentive communication layers for message passing.

In the message passing module, we utilize the \ac{HEAT} operator\cite{HEAT}.
This operator enhances the \ac{GAT} \cite{GAT} by incorporating type-specific transformations of nodes and edges features during message passing. 
Similar to \ac{GAT}, \ac{HEAT} allows running several independent attention heads to stabilize the self-attention mechanism.
The features from each attention head are concatenated as the updated output feature.
The output of the \ac{HEAT} operator is the updated node features from the neighborhood $K=1$ and number of attention heads $H=3$ concatenated.
The updated node features are passed to the edge updater module along with the encoded \textit{eta} edges.
In the edge updater module, the \textit{eta} edges are concatenated with the corresponding nodes and sent through a linear layer.

The decoder receives the \textit{eta} edges with timestamp $T$ and converts the eta feature vectors to \ac{ETA} predictions.
For \ac{DMS} methods, the naive time of arrival of all \textit{eta} edges in the dynamic layer is updated based on the \ac{ETA} prediction to reflect the new predicted state of all robots. 
For \ac{IMS} methods, the actual arrival time is used instead of the \ac{ETA} prediction. 
% Based on either the \ac{ETA} prediction in case of \ac{DMS} or the actual arrival time in case of \ac{IMS}, the naive time of arrival of all \textit{eta} edges in the dynamic layer is updated to reflect the new state of all robots.
As this is a recurrent process, this is repeated for $T=T+1$ until all \textit{eta} edges have been decoded.

As in the first layer, the second layer does not rely on a central station to process any information. However, global information is requested from a centralized station during run-time in order to gather information about all other agents in the system. While not a completely decentralized solution, it does improve scale-ability in terms of distributing the computations to each agent.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% COST SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validating time-constraints and path selection}

The validation of time-constraints and path selection is the third layer of the proposed framework. 
This layer utilizes the \ac{ETA} to evaluate time-constraints and calculate the cost of each suggested route. The layer is not only used to find a route that is feasible within a fixed time constraint but it is also used to validate the impact of the chosen route on the rest of the system by utilizing the predicted \ac{ETA} for all agents. There are various approaches that can be used to evaluate a time-constrained path since the metric to select the best path depends on the specific application scenarios.
% and select what is considered the best path, but the choice of method depends on the specific application scenario.
In this study, a path is considered invalid if one or more of the time constraints are not met. To select between the valid paths, a cost function is proposed that considers the trade-off between the buffer times on the time constraints and the predicted arrival time. The cost function is defined as follows:

\begin{equation}
cost=\sum_{i=1}^{N}{\Bigl(\max{(\textit{TC})} - (\textit{TC}_{i} - \text{eta}_i)\Bigr)^2}
\end{equation}

\noindent where $\textit{TC}$ represents the set of all the time constraints, $\textit{eta}$ is the set of predicted \ac{ETA} for all $N$ robots. The cost function is designed to maximize the buffer time between the constraint time and the predicted arrival time. At the same time, it penalizes the paths with a shorter buffer time and provides more slack for the paths with a larger buffer time. This ensures that the path selection process balances the objective of meeting the time constraints with the goal of minimizing the overall time spent to complete all tasks.

==> old_iros/related_work.tex <==
\section{Related work}
\label{sec:related_work}
% \noindent Plan for this section
% \begin{enumerate}
%     \item Traditional methods
%     \item state of the art in ETA pred
%     \item state of the art in multi-agent prediction
% \end{enumerate}
 % This section introduces the foundation of \ac{MAPF}, \ac{GNN}, and \ac{STSF} to understand further the design choices of \ac{CAMAGP}.
\subsection{Traditional \ac{MAPF} solutions}
The problem of \ac{MAPF} \cite{Mapf} involves determining a conflict-free path for each agent on a graph to reach their respective destinations. The passage of time is divided into discrete timesteps, during which each agent executes an atomic action in a synchronized manner, either moving to an adjacent node or remaining in their current location. The types of conflicts are described in \cite{Mapf}, but the ones considered in this paper are the following four conflicts: Vertex, edge, swapping, and cycle conflicts. Vertex conflicts happen when agents are in the same position at the same time. Edge conflicts happen when agents travel along or across the same edge. Swapping conflicts happen when two agents exchange positions. Cycle conflicts happen when multiple agents form a cycling movement.

% While the proposed work does not directly solve the \ac{MAPF} problem, it is tightly correlated. Its primary objective is to validate the discovered route by assuming imperfect plan execution and forecasting conflicts along the route. 
Offline path planning algorithms for the \ac{MAPF} problem are a class of solvers that first perform all computations in a single continuous interval and return a plan for the agents to follow. These plans are generated before the agents begin to move, and the agents follow the plan without any additional computation. This means that the plan cannot contain parts where agents collide. Some offline solvers, such as \ac{CBS} \cite{CBS}, aim to find optimal solutions according to a predefined cost function. However, these methods may not be able to scale up to larger systems due to the exponential growth of the search space as the number of agents increases \cite{yu2013structure}. Other offline algorithms, the \ac{HCA*}\cite{HCA*} and \ac{PIBT}\cite{PIBT}, sacrifice optimality or completeness in order to reduce computation time by using a spatiotemporal reservation table to coordinate agents and avoid collisions. 
A major weakness in offline path planning algorithms is that agents frequently have imperfect plan execution capabilities and cannot perfectly synchronize their motions, leading to frequent and time-consuming replanning \cite{ma2017overview}. This is addressed in \cite{honig2016multi}, where a post-processing framework is proposed, using a simple temporal graph to establish a plan-execution scheduler that guarantees safe spacing between robots. The framework exploits the slack in time-constraints to absorb some of the imperfect plan executions and prevent time-intensive replanning.
The work of \cite{MU} extends the method presented in \cite{M*} for a multi-agent path planner called uncertainty M* that considers collision likelihood to construct the belief space for each agent.
% In \cite{MU}, a multi-agent path planner called uncertainty M* that considers uncertainty in its path planning. The uncertainty M* plans a path through the belief space for each agent and coordinates only likely-to-collide agents using a strategy similar to the prior approach M*\cite{M*}. 
However, this does not guarantee to remove conflicts caused by imperfect plan execution, so an online path planning algorithm is commonly needed for solving these conflicts when they occur.

Online path planning algorithms are a class of solvers that compute partial solutions in real-time, allowing agents to adjust their plans as they execute them. A simple approach for online \ac{MAPF} is \ac{LRA*} \cite{LRA*}, which plans paths for each agent while ignoring other agents. Once the agents start moving, conflicts are resolved locally by constructing detours or repairs for some agents. Another notable online \ac{MAPF} solver is the \ac{WHCA*} algorithm \cite{HCA*}, which is an online variant of the \ac{HCA*} algorithm. \ac{WHCA*} uses a spatiotemporal reservation table to coordinate agents, but only reserves limited paths, splitting the problem up into smaller sections. As agents follow the partially-reserved paths, a new cycle begins from their current locations. In the traditional \ac{WHCA*}, a different ordering of agents is used in each cycle to allow a balanced distribution of the reservation table. An extension of the \ac{WHCA*} is proposed in \cite{COWHCA*}, where a priority is computed based on minimizing future conflicts, improving the success rate, and lowering the computation time. Learning-based methods for online planning are also showing promising results. In \cite{ robotics11050109}, an end-to-end online planning method is introduced, using reinforcement learning to generate safe pathing in dense environments. \cite{9424371} introduces the use of \ac{GNN} for local communication and imitation learning for learning the conflict resolution of \ac{CBS} in multi-agent environments.

\subsection{Spatio-temporal graph neural networks}
A spatio-temporal graph is a combination of spatio representing space or structural information and temporal representing time-varying information. 
Accordingly, if any system consists of a structural relationship between space and time, it can be represented as a spatio-temporal graph. These graphs can be used to design a neural network capable of handling static structures and time-varying characteristics. 
% We can define a spatio-temporal graph as a function of static structure and time-varying features:
% $$G = (V, E, X_{v(t)}, X_{e(t)})$$  
% where $G$ represents the graph, $V$ is the set of nodes, $E$ is the set of edges, $X_{v(t)}$ is the set of node-features at a given time $t$, and $X_{e(t)}$ is the set of edge-features at a given time $t$.

To work with spatio-temporal graphs, we must process a sequence of graph data to build a spatio-temporal embedding that may be used for regression, classification, clustering, or correlation prediction\cite{malla2021social}. The spatial block can be any conventional \ac{GNN} \cite{battaglia2018relational}, while the temporal block can be any approach for learning over sequences of data, such as temporal convolution\cite{temporal-conv, temporal-conv-2} or temporal attention\cite{temporal-attention}. 
Various spatio-temporal \acp{GNN}  conform to the encoding-processing-decoding paradigm \cite{GOOGLE_ETA,battaglia2018relational, keisler2022forecasting}. This paradigm enables us to accommodate the iterative nature of \ac{STSF} and pathfinding algorithms. 
Improving these alignments has been shown to improve \acp{GNN} generalization to a more diverse distribution of graphs\cite{velivckovic2019neural}.
% 

\subsection{\ac{ETA} prediction and spatio-temporal sequence forecasting}
\label{sec:IMS-vs-DMS}
% Generally, \ac{ETA} predictions fall into the category of the \ac{STSF} problem.
The \ac{STSF} problem aims to predict a sequence of length $L$ into the future based on past observations and auxiliary data. The general learning strategies for multi-step forecasting fall into two major categories: \ac{IMS} estimation and \ac{DMS} estimation\cite{forecast_survey}. The \ac{IMS} strategy trains a one-step-ahead forecasting model and iteratively feeds the generated samples to the one-step-ahead forecaster to produce a multi-step-ahead forecast.
There are two main benefits of the \ac{IMS} strategy:
the one-step-ahead forecaster is simple to train because it only needs to consider the one-step-ahead forecasting error, and it can be used to generate predictions of any length. The work of \cite{DCRNN} demonstrates how accounting for graph structure significantly reduces forecasting error across multiple horizons.
% Improving previous work, \cite{Gman} proposes the graph multi-attention network, a transform attention mechanism to transform the historical traffic features into future representations. This attention mechanism models direct relationships between historical and future time steps to alleviate the problem of error propagation.
% This design of spatial GNN combined with temporal component has yielded several subsequent proposals; STGCN\cite{STGCN}, GaAN\cite{GaAN}, ST-GRAT\cite{STGRAT}, and GMAN\cite{Gman}.
However, there is a disparity between the training and testing phase in \ac{IMS}.
In the training phase, the $L$th-step prediction is generated using the ground truths of the previous $L - 1$ steps, while in the testing phase, the model is provided with its previous prediction of the $L - 1$ steps rather than ground truths. This disparity makes the model susceptible to accumulating forecasting errors \cite{bengio2015scheduled}.

\ac{DMS} circumvent the accumulated error issue seen in \ac{IMS} by directly minimizing the long-term prediction error. Rather than training a single model, \ac{DMS} trains a distinct model $m_h$ for each forecasting horizon h. Therefore, the \ac{DMS} approach can support up to $L$ internal models. In order to separate the model size from the number of forecasting steps $L$, we can also construct $m_h$ by recursively applying the one-step-ahead forecaster $m_1$ in order to compute the multi-step-ahead forecasting error. It is worth noting that a multi-step-ahead forecasting error differs from a one-step-ahead forecasting error. Multi-step-ahead forecasting error accumulates the error during the sequence, while one-step-ahead forecasting error only minimizes for one step.
% This recursive \ac{DMS} method is widely adopted in deep learning-based methods including, Google maps\cite{GOOGLE_ETA}, Stg2seq\cite{Stg2seq}, Graph WaveNet\cite{wavenet}, and StemGNN\cite{StemGNN}.
Using \ac{DMS} does not come without cost\cite{chevillon2007direct}. \ac{DMS} is more computationally expensive than \ac{IMS}. For multi-model DMS, $L$ models need to be stored and trained, while recursive \ac{DMS} needs to apply $m_1$ for $\mathcal{O}(L)$ steps. Both cases require a large amount of memory storage or longer training time than solving the \ac{IMS} method. On the other hand, the \ac{IMS} training process is easily parallelizable since each forecasting horizon can be trained independently\cite{Goodfellow-et-al-2016}.

% Papers spatial–temporal graph neural network, GOOGLE_ETA,
In\cite{GOOGLE_ETA}, a homogeneous spatio-temporal \ac{GNN} method for predicting \ac{ETA} is proposed. While the main architecture consists of basic \ac{GNN} building blocks, they propose utilizing a combination of the recursive \ac{DMS} and multi-model \ac{DMS} to improve long horizon predictions. 
% Five models are trained using the recurrent \ac{DMS} for predicting $0$, $10$, $20$, $30$, and $60$ minutes into the futures. The model predicts the time it takes to traverse each node in the system during these five timeslots.
In \cite{huang2022dueta}, a focus on modeling traffic congestion propagation into a congestion-sensitive graph structure is proposed.
% Specifically, instead of directly using the road network as a graph, a congestion-sensitive graph based on the correlations of traffic patterns is introduced.
% In addition, a route-aware graph transformer layer is proposed to directly learn the road segment's long-distance correlations. 
In addition, a route-aware graph transformer layer is proposed enabling \acp{GNN} to capture the interactions between any road segments that are spatially distant but highly correlated with traffic conditions.
A novel heterogeneous graph structure is proposed in \cite{hong2020heteta}, which models both road features and historical data as heterogeneous information. It introduces edge features containing structural information on the relationship between nodes. In addition, three components are introduced to model temporal information from recent periods, daily periods, and weekly periods respectively. Each component comprises temporal convolutions and graph convolutions to learn representations of the spatio temporal heterogeneous information. 

% While all the above-mentioned methods generate excellent results, they focus mainly on the features of the road and consider only a single vehicle traversing the graph. None of the models consider other types of vehicles driving in the environment or how the traffic is influenced due to the driver choosing the route. As a result, such models are not easily converted into multi-vehicle solutions.

The methods mentioned above focus mainly on the features of the road and consider only a single vehicle traversing the graph. None of the models consider other types of vehicles driving in the environment or how the traffic is influenced due to the driver choosing the route. As a result, such models are not easily converted into multi-vehicle solutions.


% you should make comments and comparisons with these papers. One by one, please tell us what they have done and why it is good or bad. What is missing? and what contributions are made after this paper?

%Generally speaking, DMS is preferred for short-term prediction, where the dimensionality of data is very large, and only short-term predictions are required [5], [6]. IMS is preferred for long-term forecasts where the forecasting horizons are long, which are generally above 12 [4], [13] and can be as long as 100 [14].

% \textcolor{red}{Google maps example}
% When looking into how \ac{GNN} \cite{GOOGLE_ETA}



% Mapper
% Graph Neural Networks for Decentralized Multi-Robot Path Planning

==> old_iros/results.tex <==
\input{LargeObjects/ETAResultTable.tex}
% \input{LargeObjects/CostResultTable.tex}
\section{Results}
\label{sec:results}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{images/Results/final_250.png}
%     \caption{The absolute errors are plotted over the path length for the three \ac{DMS} models on the 250 robot test dataset. The shaded areas are the standard deviation over and under the mean absolute error for each of the three models.}
%     \label{fig:length-comparison}
% \end{figure}
% \begin{enumerate}
    % \item (Table) Compare DMS, IMS, and naive (All the loss functions) \ref{table:comparison}. 
    % \item (Graph) Prediction error over the length of the path.
    % \item (Graph) Prediction error over the number of robots.
% \end{enumerate}
% \begin{figure*}
%     \centering
%     % \begin{subfigure}[b]{0.2\textwidth}
%     %      \centering
%     %      \includegraphics[width=\textwidth]{images/Results/paper_448x448_3.png}
%     %     %  \caption{The plot shows the increase in sum of costs as noise is applied in various degrees.}
%     %      \label{fig:socs}
%     % \end{subfigure}
%     % \vspace*{\fill}
%     %  \hfill
%     \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/Results/noise_soc_results-1.pdf}
%         %  \caption{The plot shows the increase in sum of costs as noise is applied in various degrees.}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/Results/noise_makespan_results-1.pdf}
%         %  \caption{The plot shows the increase in makespan as noise is applied in various degrees.}
%      \end{subfigure}
    
%     \caption{The two plots illustrates the results of noise in various degrees can greatly affect both sum of costs and makespan.}
%     \label{fig:noise-results}
% \end{figure*}

\subsection{Estimate time of arrival prediction}
\subsubsection{Method comparisons}
The first experiment compares the performance of the naive method, which does not use conflict-aware correction, the \ac{IMS} method, and the \ac{DMS} method. As shown in Table \ref{table:comparison}, using conflict-aware correction with either \ac{IMS} or \ac{DMS} significantly reduces error.
It can be seen that the \ac{DMS} methods perform better than \ac{IMS} methods due to the accumulated error nature in \ac{IMS},
% Comparing the \ac{IMS} and \ac{DMS} methods, it is clear that the \ac{DMS} method is able to learn more from the training data. It is due to the accumulated error issue in \ac{IMS},
as explained in Section \ref{sec:IMS-vs-DMS}. There is a disparity between the training and testing phases, and as the density of robots rises and more conflict happens in the environment, the harder it is for the \ac{IMS} method to adapt to incorrect predictions. The best trained \ac{IMS} model improves the average \ac{MAPE} by 29.5$\%$ compared to the naive method, while the best \ac{DMS} model improves by 44$\%$. 

% The second experiment demonstrates the relationship between prediction error and path length. As depicted in Fig. \ref{fig:length-comparison},  the prediction error generated by multi-step prediction methods accumulates in proportion to the path length. Since each prediction is based on the previous prediction, the standard deviation increases rapidly as the number of prediction iterations increases. Around the path length of $175$, the error curve plateau due to less number of robots moving, and hereby less conflict occurs. The standard deviation under the \ac{MAE} curve is smaller compared to above the curve. This depicts that the majority of the predictions lie beneath the \ac{MAE} curve with a smaller error. Contrarily, the standard deviation over the \ac{MAE} curve lies farther away, indicating that the model does not accurately predict a fewer number of paths, therefore generating big standard deviation errors.

% Since the three models have roughly the same curve structure, it seems the dataset could contain some outliers that all models are having trouble predicting.

\subsubsection{Generalization under different robot densities}
The second experiment demonstrates the generalization of the models in environments of varying densities. This is highly pertinent given that the number of robots can vary based on the season, demand, and business case. Therefore, for the industry to freely add or remove robots without retraining, the generalization across densities is of great importance.
As shown in Table \ref{table:comparison}, three different models trained on a dataset containing $250$, $500$, and $1000$ robots are compared at different densities. The results indicate that training in environments of high density generalizes well to environments of low density. This implies that none of the models are overfitting to any density-specific features in the graph representation. 

The \ac{DMS} models trained with the same number of robots as in the test scenario generally perform slightly better, as depicted in bold in Table. \ref{table:comparison}. However, in the $500$ robot test environment, the $1000$ robot \ac{DMS} model outperforms the $500$ robot \ac{DMS} model in terms of \ac{RMSE}. As more conflicts are happening in higher density environments, the $1000$ robot \ac{DMS} model is generally trained on paths much longer compared to the $500$ robot \ac{DMS} model. As a result, since \ac{RMSE} is sensitive to longer paths as they are accumulating more errors, as shown in experiment two, the $1000$ robot \ac{DMS} is better suited for outliers occurring within the $500$ robot test dataset.
The last column of Table \ref{table:comparison} shows average results in all the test environments. The \ac{DMS} model trained on $1000$ robots has proven to be the most generalized model.

\subsection{Evaluation of the offline path planners}

\begin{figure}[t]
   \centering
   \includegraphics[width=0.49\textwidth]{images/Results/noise_makespan_results.pdf}
   \caption{The plot shows the increase in makespan as noise is applied in various degrees. As the cost function priorities the agents with the tightest schedule, a stable makespan can be seen for \ac{CAMETA}.}
   \label{fig:noise-results-makespan}
\end{figure}
\begin{figure}[t]
   \centering\includegraphics[width=0.49\textwidth]{images/Results/noise_soc_results.pdf}
   \caption{The plot shows the increase in sum of costs as noise is applied in various degrees. Both \ac{PIBT} and \ac{CBS} rises as the noise increases, while $A^*$ and \ac{CAMETA} is less affected by the noise.}
   \label{fig:noise-results-soc}
\end{figure}
% The results of the path planners under the influence of noise are presented in Fig. \ref{fig:noise-results-makespan} and Fig. \ref{fig:noise-results-soc}. The \ac{CBS} method yielded the optimal solution at a noise level of $0\%$, which highlights the disparity between this method and the real-time counterparts. While the \ac{CBS} algorithm demonstrates superior performance in terms of \ac{SOC} compared to other methods, its computational time was extremely long, taking four hours to generate the optimal solution.

% The \ac{CAMETA} and \ac{PIBT} methods yielded comparable results at $0\%$ noise, with \ac{CAMETA} outperforming \ac{PIBT} by utilizing the exploration of alternative paths with fewer conflicts. In contrast, \ac{PIBT} only resolved conflicts based on the $A^*$ algorithm, incorporating 'wait' actions and priority inheritance. 
% The basic $A^*$ method yielded the poorest results at this noise level, as expected, due to the lack of conflict resolution in the planning.

% As the noise level increased, \ac{PIBT} demonstrated a decrease in performance due to the coordinated nature of its planned paths, which left little room for error. The additional moves planned for conflict resolution did not align with the expected conflicts, leading to the generation of even more conflicts, resulting in a rapid increase in total moves required to resolve everything as the noise level increased. This is reflected in Fig. \ref{fig:noise-results-soc} as a rapid increase in \ac{SOC} for the \ac{PIBT} method. The online planner, \ac{WHCA*}, took over to resolve conflicts as the noise level increased. However, due to the extra moves already planned for conflicts, conflicts arising from noise were harder to resolve.

% Both the basic $A^*$ and \ac{CAMETA} methods demonstrated a stable pattern as the noise level increased, as they relied on conflicts being resolved in real-time, making it easier for the online planner to correct. However, \ac{CAMETA} exhibited much better overall results in terms of total \ac{SOC} and makespan, as it reduced the number of conflicts by allowing for longer routes and distributing traffic, resulting in noise not affecting the planned path as much.

% Overall, the results suggest that while \ac{CBS} may provide the optimal solution in terms of \ac{SOC}, it is not a feasible solution for real-time applications. On the other hand, \ac{CAMETA} exhibits more promising and stable performance in terms of real-time path planning under noisy conditions.


The results of the path planners under the effect of noise are presented in Fig. \ref{fig:noise-results-makespan} and Fig. \ref{fig:noise-results-soc}. The \ac{CBS} method yields the optimal solution at a noise level of $0\%$, which highlights the disparity between this method and the real-time counterparts. While the \ac{CBS} algorithm demonstrates superior performance in terms of \ac{SOC} compared to other methods, its computational time is extremely long, taking four hours to generate the optimal solution.

The \ac{CAMETA} and \ac{PIBT} methods yield comparable results at $0\%$ noise, with \ac{CAMETA} outperforming \ac{PIBT} by utilizing the exploration of alternative paths with fewer conflicts. In contrast, \ac{PIBT} only resolves conflicts based on the $A^*$ algorithm, incorporating 'wait' actions and priority inheritance.
The basic $A^*$ method yields the poorest results at this noise level, as expected, due to the lack of conflict resolution in the planning. As the noise level increases, \ac{PIBT} demonstrates a decrease in performance due to the coordinated nature of its planned paths, which leaves little room for error. The additional moves planned for conflict resolution do not align with the expected conflicts, leading to even more conflicts, resulting in a rapid increase in total moves required to resolve everything as the noise level increases. This is reflected in Fig. \ref{fig:noise-results-soc} as a rapid increase in \ac{SOC} for the \ac{PIBT} method. The online planner, \ac{WHCA*}, resolves conflicts as the noise level increases. However, due to the extra moves already planned for conflicts, conflicts arising from noise are harder to resolve.

Both the basic $A^*$ and \ac{CAMETA} methods demonstrate a stable pattern as the noise level increases, as they rely on conflicts being resolved in real-time, making it easier for the online planner to correct. However, \ac{CAMETA} exhibits better results in terms of total \ac{SOC} and makespan, as it reduces the number of conflicts by allowing for longer routes and distributing traffic, resulting in noise not affecting the planned path as much.

Overall, the results illustrate that while \ac{CBS} may provide the optimal solution in terms of \ac{SOC}, it is not a feasible solution for real-time applications. On the other hand, \ac{CAMETA} exhibits more promising and stable performance in terms of real-time path planning under noisy conditions.
